SWATI: Synthesizing Wordlengths Automatically Using Testing and Induction

In this paper, we present an automated technique SWATI: Synthesizing Wordlengths Automatically Using Testing and Induction, which uses a combination of Nelder-Mead optimization based testing, and induction from examples to automatically synthesize optimal fixedpoint implementation of numerical routines. The design of numerical software is commonly done using floating-point arithmetic in design-environments such as Matlab. However, these designs are often implemented using fixed-point arithmetic for speed and efficiency reasons especially in embedded systems. The fixed-point implementation reduces implementation cost, provides better performance, and reduces power consumption. The conversion from floating-point designs to fixed-point code is subject to two opposing constraints: (i) the word-width of fixed-point types must be minimized, and (ii) the outputs of the fixed-point program must be accurate. In this paper, we propose a new solution to this problem. Our technique takes the floating-point program, specified accuracy and an implementation cost model and provides the fixed-point program with specified accuracy and optimal implementation cost. We demonstrate the effectiveness of our approach on a set of examples from the domain of automated control, robotics and digital signal processing.

==> Makefile <==
# Makefile

# Set this to the basename of the .tex file
# This will also be the name of the generated .dvi, .ps and .pdf files
PAPER = main

# Set this to the other source files that should be counted as 
# dependencies
OTHERSOURCES := main.tex
 
# Set this to the basenames of the files containing figures
# !!! If you do not want to regenerate the figures, run "make FIGURES="
FIGURES = 


.PHONY: ps
ps: $(PAPER).ps

.PHONY: pdf
pdf: $(PAPER).pdf




# run once, then re-run until it's happy
# input redirected from /dev/null is like hitting ^C at first error
$(PAPER).dvi: $(PAPER).tex $(OTHERSOURCES) $(FIGURES:%=%.eps)
	if latex $(PAPER).tex </dev/null; then \
		true; \
	else \
		stat=$$?; touch $(PAPER).dvi; exit $$stat; \
	fi
	bibtex $(PAPER)
	while grep "Rerun to get" $(PAPER).log; do \
		if latex $(PAPER).tex </dev/null; then \
			true; \
		else \
			stat=$$?; touch $(PAPER).dvi; exit $$stat; \
		fi; \
	done

$(PAPER).pdf: $(PAPER).dvi $(FIGURES:%=%.pdf) 
# Remove the .aux file because pdflatex wants it different
	rm -f $(PAPER).aux 
	if pdflatex $(PAPER).tex </dev/null; then \
		true; \
	else \
		stat=$$?; touch $(PAPER).pdf; exit $$stat; \
	fi
	bibtex $(PAPER)
	while grep "Rerun to get" $(PAPER).log; do \
		if pdflatex $(PAPER).tex </dev/null; then \
			true; \
		else \
			stat=$$?; touch $(PAPER).pdf; exit $$stat; \
		fi; \
	done

$(PAPER).ps: $(PAPER).dvi
	dvips -tletter -o $(PAPER).ps $(PAPER).dvi


clean:
	rm -f *.aux *.log *.ps *.dvi *.blg *.bbl *.toc *~ *.out *.pdf 
	#no eps files here - take from thesis

# Generate PDF figures from the EPS ones
%.pdf: %.eps
	epstopdf $<



==> exp.tex <==
\section{Experiments} \label{icse12:sec:exp}

We present case-studies from DSP and control systems to illustrate
the utility of the presented synthesis approach.
 
\subsection{Infinite Impulse Response (IIR) Filter}


The first case study is an IIR filter which is used
in digital signal processing applications.
It is a first-order direct form-II IIR filter with
the schematic shown in Figure~\ref{fig:fx:iir}.
The constants are $a_1 = -0.5$, $b0 = 0.9$ and $b1 = 0.9$.
The fixed-point variables are identified in the schematic.
We use our synthesis technique to discover the appropriate 
fixed-point types of these variables. 
The input domain used in synthesis is $-2 < input < 2$.
The correctness condition for accuracy is to ensure that the relative 
error between the floating-point and fixed-point program is less 
than $0.1$.
We use the  Constantinides et al~\cite{constantinides-FCCM02} 
cost model.
%The obtained
%fixedpoint types are shown in Table~\ref{tbl:fx:iir}.


\begin{figure}[ht]
\centering
\includegraphics[width=5in]{iir}
\caption{IIR Filter Schematics}
\label{fig:fx:iir}
\end{figure}


\noop{
\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
\caption{Synthesized Fixed-point Types for IIR Filter}
\label{tbl:fx:iir}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Variables & a1 & b0 & b1 & t1 &  t3  \\
\hline
Fixed-point Types &  $\langle 1,2,1  \rangle$  &  $\langle 0,1,5  \rangle$ & $\langle 0,1,3  \rangle$ &  $\langle 1,2,6  \rangle$ &  $\langle 1,2,4  \rangle$  \\
\hline
Variables & t4 & t5 & t6 & t7 & t8 \\
\hline
Fixed-point Types &  $\langle 1,3,5  \rangle$ &  $\langle 1,3,5  \rangle$ &  $\langle 1,3,5  \rangle$ &  $\langle 1,3,6  \rangle$ &  $\langle 1,4,6  \rangle$ \\
\hline
\end{tabular}
\end{table}
}


\begin{figure}[ht]
\centering
\includegraphics[width=6in]{iirsim}
\caption{IIR Filter Using Floating-point and Fixed-point}
\label{fig:fx:iirsim}
\end{figure}



In order to test the correctness of our implementation,
we feed a common input signal to both the IIR filter implementations:
floating-point version and the fixed-point version obtained by our 
synthesis technique. 
The input signal is a linear chirp from $0$ to $\frac{Fs}{2}$ Hz in $1$ second.
$$input = (1-2^{-15}) \times sin(\pi \times \frac{Fs}{2}\times t^2)$$
where $Fs = 256$  and $t=0$ to $1-\frac{1}{Fs}$ and is
sampled at intervals of $\frac{1}{Fs}$.
Figure~\ref{fig:fx:iirsim} shows the
input, 
outputs of both implementations and the relative error
between the two outputs. We observe that the implementation
satisfies the correctness condition and the relative error 
remains below $0.1$ throughout the simulation.


\subsection{Field Controlled DC Motor}

The next case study is a field controlled DC Motor. 
It is a classic non-linear control example from 
Khalil~\cite{khalil-book}. The example used here is an adaptation of 
Khalil's example presented in \cite{claire-course}.
The system dynamics is described by the following ordinary differential
equations.
\begin{align*}
\dot v_f = R_fi_f + L_f \dot i_f\\
\dot v_a = c_1 i_f \omega + L_a \dot i_a + R_a i_a \\
\dot J \dot \omega = c_2 i_f i_a - c_3 \omega
\end{align*}

The first equation is for the field circuit with $v_f, i_f, R_f, L_f$ 
being its voltage, current, resistance, and inductance. 
The variables $v_a, i_a, R_a, L_a$ are the corresponding 
 voltage, current, resistance, and inductance
of the armature circuit described by the second equation.
The third equation is a torque equation for the shaft, with
$J$ as the rotor inertia and $c_3$ as a damping coefficient. 
The term $c_1 i_f \omega$ is the back electromotive force induced in 
the armature circuit, and $c_2 i_f i_a$ is the torque produced by the 
interaction of the armature current with the field circuit flux.
In the field controlled DC motor, 
field voltage $v_f$ is the control input while $v_a$ is held constant.
The purpose of the control is to drive the system 
to the desired set point for the angular velocity $\omega$. 

We can now rewrite the system dynamics in the following normal 
form where $a = \frac{R_f}{L_f}$, $u = \frac{ v_f}{L_f}$, $b = \frac{R_a}{L_a}$,
$\rho =  \frac{v_a}{L_a}$, $c = \frac{c_1}{L_a}$, 
$\theta = \frac{c_2}{J}$, $d = \frac{c_3}{J}$.
\begin{align*}
 \dot i_f = - a i_f + u \\
 \dot i_a =  - b i_a  + \rho - c i_f \omega \\
 \dot \omega = \theta i_f i_a - d \omega
\end{align*}
We assume no damping, that is, $c_3 = 0$ and set all the other
constants $a,b,c,\theta,\rho$ to $1$~\cite{claire-course}.
The state feedback law to control the system is given by
$$ u = \frac{\theta(a+b)i_f i_a + \theta \rho i_f - c \theta i_f^2 \omega}{\theta i_a + \epsilon}$$
where $\epsilon = 0.01$ is added to denominator to avoid division by $0$. $i_a$
approaches $0$ at equilibrium.
 The system is initialized with 
field current $i_f = 1$, armature current $i_a = 1$ 
and angular velocity $\omega = 1$. 



\begin{figure}[ht]
\centering
\includegraphics[width=6in]{DCmotor-Fixed-point}
\caption{DC Motor Using Floating-point and Fixed-point Controller}
\label{fig:fx:dcmotorfx}
\end{figure}


The computed control law can be mathematically shown to be 
correct by designers who are more comfortable in reasoning with
real arithmetic but not with finite precision arithmetic. 
Its implementation using floating-point computation
also closely mimics the arithmetic in reals
 but the control algorithms are often implemented using
fixed-point computation on embedded platforms.
This reduces power consumption and allows the use of cheaper processors.
In this case study, we use our synthesis technique to automatically
derive a low cost fixed-point implementation of the control law
computing $u$.
The input domain is $0 \leq i_a,i_f,\omega \leq 1.5$.
The correctness condition for accuracy is that the absolute
difference between the $u$ computed by fixed-point program and the 
floating-point program is less than $0.1$. 

Figure~\ref{fig:fx:dcmotorfx} shows the simulation of the system
using the fixed-point implementation of the controller
and the floating-point implementation. 
This end-to-end
simulation shows that fixed-point program generated by our technique 
can be used to control the system as effectively as the floating-point program.
This illustrates the practical utility of our technique. 
Figure~\ref{fig:fx:dcmotoru} shows how the control input 
computed by fixed-point and the floating-point are 
close to each other.
Figure~\ref{fig:fx:motorerror} plots the difference between
the two. It clearly
shows that the correctness condition is satisfied and the
difference between the control input computed by 
the fixed-point and floating-point program is within 
the specified maximum error threshold of $0.1$.


\begin{figure}[ht]
\centering
\subfigure[Computed Control Input]
{
\includegraphics[width=3.1in]{DCmotor-u}
\label{fig:fx:dcmotoru}
}
\subfigure[Error]
{
\includegraphics[width=3.1in]{dcmotor-error}
\label{fig:fx:motorerror}
}
\caption{Control Input Using Fixed-point and Floating-point Program}
\end{figure}

\subsection{Two-Wheeled Welding Mobile Robot}

The next case-study is a nonlinear controller for a two-wheeled welding 
mobile robot (WMR)~\cite{bui-jcas03,dung-jcas07}. The robot consists of
two wheels and a robotic arm. The wheels can roll and there is no slipping.
$(x,y)$ represents the Cartesian coordinate of the WMR's center point
and $\phi$ is the heading angle of the WMR. $v$ and $\omega$ are the straight
and angular velocities of the WMR at its center point. 
The welding point coordinates $(x_w, y_w)$ and the heading angle $\phi_w$
can be calculated from the WMR's center point:
\begin{align*}
x_w = x - l \sin\phi\\
y_w = y + l \cos\phi\\
\phi_w = \phi
\end{align*}
So, the equation of motion for the welding point is as follows:
\begin{align*}
\dot x_w = v \cos\phi - l \omega \cos\phi - \dot l \sin\phi\\
\dot y_w = v \sin\phi - l \omega \sin\phi + \dot l \cos\phi\\
\dot \phi_w = \omega
\end{align*}

The objective of the WMR controller is to ensure that the robot
tracks a reference point R. 
The reference point R moving with a constant velocity
of $v_r$ on the reference path has coordinates
$(x_r, y_r)$ and the heading angle $\phi_r$.
The tracking error is the difference between the location of 
the robot and the reference point. 


\[
\left[ {\begin{array}{c}
 e_1 \\
 e_2 \\
 e_3
\end{array} } \right]
= 
\left[ {\begin{array}{ccc}
 \cos\phi & \sin\phi & 0 \\
 -\sin\phi & \cos\phi & 0 \\
 0 & 0 & 1 \\
\end{array} } \right] 
\left[ {\begin{array}{c}
 x_r - x_w \\
 y_r - y_w \\
 \phi_r - \phi_w
\end{array} } \right]
\]


The two control parameters in the model are $v$ and $\omega$.
In order to ensure that the error quickly converges to $0$,
a nonlinear controller based on Lyapunov stability is
as follows:
\begin{align*}
v = l(\omega_r + k_2 e_2 v_r + k_3 \sin e_3) + v_r \cos e_3 + k_1 e_1\\
\omega = \omega_r + k_2 e_2 v_r + k_3 \sin e_3
\end{align*}
where $k_1, k_2$ and $k_3$ are positive constants. 
Table~\ref{tbl:fx:mwrval} provides
the numerical values of constants and initial values of the
state variables from Bui et al~\cite{bui-jcas03}.
All lengths are in meters, angle in radians and time in seconds.

\begin{table}[!h]
\caption{Numerical and Constant Values}
\label{tbl:fx:mwrval}
\centering
\begin{tabular}{|c|c||c|c|}
\hline
Parameters & Values & Parameters & Values  \\
\hline
$k_1$ & $4.2$ & $l$ & $0.15$ \\
$k_2$ & $5000$ & $\dot l$ & $0$ \\
$k_3$ & $1$ & $v_r$ & $7.5e-3$\\
\hline
$x_r$ & $0.280$ & $x_w$ & $0.270$ \\
$y_r$ & $0.400$ & $y_w$ & $0.390$ \\
$\phi$ & $0$ & $\phi_w$ & $15$\\
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=6in]{WMRreference}
\caption{Reference Welding Line}
\label{fig:fx:WMRref}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=6in]{distance}
\caption{Distance of WMR from Reference Line}
\label{fig:fx:WMRdist}
\end{figure}


\noop{
\begin{figure}[h]
\centering
\subfigure[Reference Welding Line]
{
\includegraphics[width=3.1in]{WMRreference}
\label{fig:fx:WMRref}
}

\subfigure[Distance of WMR from Reference Line]
{
\includegraphics[width=3.1in]{distance}
\label{fig:fx:WMRdist}
}
\caption{Welding Motor Robot}
\end{figure}
}



\begin{figure}[!h]
\centering
\includegraphics[width=6in]{errorv}
\caption{Error in computing $v$}
\label{fig:fx:WMRerrorv}
\end{figure}

\begin{figure}[!h]
\centering
\includegraphics[width=6in]{erroromega}
\caption{Error in computing $\omega$}
\label{fig:fx:WMRerroromega}
\end{figure}


We use our synthesis technique to automatically synthesize fixed-point
program for both control inputs: $v$ and $\omega$. 
The error function used for $v$ is the relative difference
$$\frac{v_{floating-point} - v_{fixed-point}}{v_{floating-point}}$$
and the error function used for $\omega$ is the moderated
relative difference
$$\frac{\omega_{floating-point} - \omega_{fixed-point}}{\omega_{floating-point}+\delta}$$
where $\delta = 0.001$. The moderated relative difference is useful here
since $\omega_{floating-point}$ can be $0$.
We require that the difference values for both controllers 
are less than $0.1$.
Figure~\ref{fig:fx:WMRref} shows the reference line for welding 
and Figure~\ref{fig:fx:WMRdist} shows the distance of the WMR from the
reference line as a function of time for both cases: firstly, when
the controller is implemented as a floating-point program and secondly,
when the controller is implemented as a fixed-point program synthesized
using our technique.
The robot starts a little away
from the reference line but quickly starts tracking the line in both
cases. Figure~\ref{fig:fx:WMRerrorv} and Figure~\ref{fig:fx:WMRerroromega}
show the error between the floating-point
controller and fixed-point controller for both control inputs: $v$ and $\omega$,
respectively. 


==> localintroprelprobdef.tex <==

\section{Introduction} 

Numerical computation with specified accuracy is of fundamental
importance in many applications such as digital signal processing and
control systems. Algorithms for these applications are often designed 
ignoring the finite precision of computer arithmetic. Quantization
errors due to finite precision are analyzed later. Floating-point
environments are very useful in providing a convenient design
and validation environment to designers who can use it to explore
the algorithm space and also quickly simulate the design using
standard floating-point units available on computers. When these algorithms
need to be implemented on hardware,  floating-point data types
are converted to fixed-point data types in order to reduce the cost
of hardware needed as well as to decrease the power requirement
and increase the speed of computation. 
The conversion from floating-point
to fixed-point often results into decreased computation
accuracy. An optimal selection of word-lengths
of fixed-point variables to ensure accuracy remains above the 
specified threshold and the implementation cost is low, 
is a challenging task.

Along with a floating-point implementation of numerical
computation, the user can provide additional specification
regarding the desired fixed-point implementation.
The floating-point program takes inputs from a given {\em input domain}.
This input domain can be provided as a logical condition on the
inputs.
Numerical computation is expected to have some
{\em specified threshold of numerical accuracy}
which can be provided as a correctness condition for the fixed-point
program.
Further, the fixed-point implementation has a cost associated
with it and an optimal implementation is
expected to take minimal cost. 
The user can provide a cost model for the implementation.
In this paper, we present an automated approach to synthesize
optimal fixed-point implementation from floating-point code
that satisfies the correctness condition and is of minimal cost.
PAPER ORGANISATION IF SPACE PERMITS

\section{Preliminaries}

Floating-point~\cite{goldberg-ACM91} is a system for 
approximately representing real numbers
which supports a wide range of values. It allows the use
of a fixed number of significant digits which is scaled using
an exponent to represent real numbers approximately.
The floating-point system is so called because
the radix point can {\em float} anywhere relative to the
significant digits of the number. 
In contrast to fixed-point numbers, floating-point
representation can be used to support a much wider range of 
values with the same number of digits. 
The most common
floating-point representation used in computers is
that defined by IEEE 754 Standard~\cite{IEEE754}. 

In order to support floating-point programs, the
{\em IMP} programming language needs to be augmented with
single-precision and double-precision floating types
as defined in IEEE 754 Standard. 
The storage layout of the floating-point numbers consist of
three basic components: 
the sign, the exponent, and the mantissa.
The storage layout of the single-precision and double-precision floating
point numbers is presented in Table~\ref{prog:prel:floatlayout} 
\begin{itemize}
\item
The {\em sign bit} is $0$ for a positive number and $1$ for 
a negative number. Flipping the value of this bit flips the sign of the number. 
\item 
The {\em mantissa}, also known as the significand, represents the precision 
bits of the number. It is composed of an implicit leading bit and the 
fraction bits.
In order to maximize the quantity of representable numbers, floating-point 
numbers are typically stored with the radix point after the first non-zero 
digit. In base $2$, the only possible non-zero digit is $1$.
Thus, we can just assume a leading digit of 1, and don't need to represent 
it explicitly. As a result, the mantissa has effectively $24$ bits of 
resolution, by way of $23$ fraction bits in single-precision floating-point 
numbers, and $53$ bits of resolution, by way of $52$ fractional bits in
double-precision.
\item 
The {\em exponent} 
field needs to represent both positive and negative exponents. 
To do this, a bias is added to the actual exponent in order to get the 
stored exponent. For IEEE single-precision floats, this value is $127$. 
Thus, an exponent of $0$ means that $127$ is stored in the exponent field. 
A stored value of $200$ indicates an exponent of $(200-127)$, or $73$. 
Exponents of $-127$ (all $0$s) 
and $+128$ (all $1$s) are reserved for special numbers.
For double precision, the exponent field is $11$ bits,
 and has a bias of $1023$. 
\end{itemize}

\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
& Sign & Exponent & Fraction & Bias \\
\hline
Single Precision & $1 \;[31]$ & $8 \;[30-23]$ & $23 \;[22-00]$ & $127$ \\
\hline
Double Precision & $1 \;[63]$ &	$11 \;[62-52]$ & $52 \;[51-00]$ & $1023$\\
\hline
\end{tabular}
\caption{Floating-point Number Layout}
\label{prog:prel:floatlayout}
\end{table}

Floating-point solves a number of representation problems. 
Fixed-point has a fixed window of representation, which limits 
it from representing very large or very small numbers. 
Floating-point, on the other hand, employs a sort of 
``sliding window'' of precision appropriate to the scale of the number. 
The range of positive floating-point numbers can be split into 
normalized numbers (which preserve the full precision of the mantissa), 
and denormalized numbers.
The denormalized
numbers do not have an implicit leading bit of $1$ and
allow representation of really small numbers but with
only a portion of the fraction's precision.
The exponent of all $0$s ($-127$) and all $1$s ($128$) 
are reserved for denormalized numbers and 
representing infinity respectively. 
A complete discussion on the semantics of floating-point
operations can be found in the
 IEEE 754 Standard~\cite{IEEE754}. 


A floating-point unit (FPU) is used to carry out
operations on floating-point numbers such as addition, subtraction,
multiplication, division and square root. Some floating-point 
operations such as exponential and trigonometric calculation
could be emulated in a software library routine or supported
explicitly by FPUs. The latter is more common with modern FPUs.
FPUs are integrated with CPUs in computers but most embedded
processors do not have hardware support for floating-point
operations. Emulation of floating-point operations
without hardware support can be very slow. The high cost of FPUs
make it prohibitively expensive to include them in many low cost 
embedded systems.
Inclusion of FPUs also increases the power consumption of the processors.
This has made the use of fixed-point arithmetic very common in
embedded systems.

Fixed-point~\cite{yates-09} is a system for representing real numbers 
in which there are fixed number of digits and the radix point
is also fixed. Fixed-point data consists of a sign mode bit,
an integer part and a fractional
part. We denote the fixed-point type of a variable $x$ by $\fxtype(x)$. 
A fixed-point type is a $3$-tuple.
$$\langle \signbit, \iwl, \fwl \rangle$$
The sign mode bit $\signbit$ is $0$ if the data is unsigned and is $1$ if the
data is signed.
The number of bits used for representing integers 
is called the integer wordlength ($\iwl$) and the number of bits used 
for representing 
fraction is called the fractional wordlength ($\fwl$).
The fixed-point wordlength
($\wl$) is the sum of the integer wordlength 
and fractional wordlength, that is, $\wl = \iwl + \fwl$.
We denote the wordlength of a variable $x$ by $\wl(x)$,
its integer wordlength by $\iwl(x)$, 
and its fractional wordlength by $\fwl(x)$. 
A fixed-point number with fractional word length ($\fwl$)
is scaled by a factor of $\frac{1}{2^{\fwl}}$. 
For example, a fixed point number $01110$ 
with $0$ as sign mode bit, integer wordlength of 2
and fractional wordlength of 2 represents $14\times \frac{1}{2^{2}}$,
that is, $3.5$.  
Converting a fixed-point number with scaling 
factor R to another type with scaling factor S, 
requires multiplying the underlying integer by R
and dividing by S; that is, multiplying by the ratio R/S. 
For example, converting $01110$ 
with $0$ as sign-bit, integer wordlength of 2
and fractional wordlength of 2 into a fixed-point
number with $0$ as sign-bit, integer wordlength of 2
and fractional wordlength of 3 requires
multiplying with $\frac{2^3}{2^{2}}$ to obtain
$011100$. If the scaling factor is to be reduced,
the new integer will have to be rounded. For example,
converting the same fixed-point number $01110$ 
to a fixed-point number with fractional wordlength
of $0$ and integer wordlength of $2$ yields
$011$, that is, $3$ which is obtained by rounding down
from $3.5$. 
The operations supported by fixed-point arithmetic
are the same as floating-point arithmetic standard~\cite{IEEE754}
but the semantics might be different on custom hardware.
For example, the rounding mode for arithmetic 
operations could be different, and the 
result could be specified to saturate or overflow/underflow
in case the wordlength of a variable is not sufficient to store
a computed result. A complete semantics of
fixed-point operation is provided with the Fixed-point Toolbox
in Maltab~\cite{fixed-matlab}.
The range of the fixed-point number is much smaller compared
to the range of floating-point numbers for the same number
of bits since the radix point is fixed and no dynamic 
adjustment of precision is possible. For example, let us
consider fixed-point numbers with $32$ bits. 
Table~\ref{prog:prel:fxrange} shows the comparison
of range of fixed-point numbers with different integer wordlengths
and fractional wordlengths, and the range of the normalized
single-precision floating-point
numbers.

\begin{table}
\centering
\begin{tabular}{|c|c|c|}
\hline
Number systems with $\wl = 32$  & Range & Precision\\
\hline
\hline
Single-precision Floating-point &  $\pm$ $ ~10^{-44.85}$ to $~10^{38.53}$ & {\em Adaptive}\\
\hline
Fixed-point type: $\langle 1, 8, 24 \rangle$& $~$ $-10^{2.11}$ to $10^{2.11}$ &  $~10^{-7.22}$  \\
\hline
Fixed-point type: $\langle 1, 16, 16 \rangle$ &  $~$ $-10^{4.52}$ to $10^{4.52}$ & $~10^{-4.82}$ \\
\hline
Fixed-point type: $\langle 1, 24, 8 \rangle$ &   $~$ $-10^{6.93}$ to $10^{6.93}$ & $~10^{-2.41}$  \\
\hline
\end{tabular}
\caption{Range of $32$ bit fixed-point and floating-point numbers}
\label{prog:prel:fxrange}
\end{table}

Thus, translating a floating-point code into fixed-point code
is non-trivial and requires careful consideration of loss of precision
and range. The integer wordlengths and fractional wordlengths of 
the fixed-point variables need to be carefully selected to ensure computation
does not loose accuracy beyond the specified threshold. 

\noop{In Chapter~\ref{fpfx}, we present an automated synthesis technique
to derive fixed-point code from floating-point code.
Fixed-point arithmetic is performed on custom hardware
and FPGA is often a natural choice for implementing 
these algorithms.
}




\section{Problem Definition} \label{icse12:sec:probdef}

We use a simple illustrative example to explain the
problem of synthesizing optimal fixed-point program
from floating-point program, and then present the formal
problem definition.

\subsection{Floating-point Implementation}
Floating-point implementation of the numerical
computation provides the scaffold of the
fixed-point program. Each floating-point variable
needs to be translated to fixed-point datatype.
 and hence,
the synthesis task is that of discovering the 
appropriate wordlength of the fixed-point variables
such that the correctness criteria is met for all
inputs satisfying the input condition and the
implementation cost is minimized.\\
\\
\noindent \textbf{Example 4.1:} 
%\begin{example}
We present an example in Procedure~\ref{icse12:proc:ch1:fpcircle}
that illustrates this problem and the
difficulty that programmers face in doing the floating-point to 
fixed-point translation manually. The floating-point
program in this example takes $\mathtt{radius}$ as the input, and
computes the $\mathtt{area}$ of the circle with this $\mathtt{radius}$.

\begin{algorithm}
\caption{Floating-point program to compute area of circle}
\label{icse12:proc:ch1:fpcircle}
\begin{algorithmic} [style=tt]
\REQUIRE $\mathtt{radius}$
\ENSURE $\mathtt{area}$
\STATE \textbf {double} $\mathtt{mypi, radius, t, area}$
\STATE $\mathtt{mypi=3.14159265358979323846}$ 
\STATE $\mathtt{t=radius \times radius}$  
\STATE $\mathtt{area=mypi \times t}$
\RETURN $\mathtt{area}$
\end{algorithmic}
\end{algorithm}


From the provided floating-point program, it is
easy to extract the scaffold of the fixed-point
program. The only unknowns are the
fixed-point type of the variables $\mathtt{mypi, radius, t}$
and $\mathtt{area}$. So, the scaffold fixed-point
program takes as input both the radius and the wordlengths
for the fixed-point variables. 
Recall that the fixed-point
type is a 3-tuple  
$\mathtt{\langle s_j,iwl_j,fwl_j \rangle}$ for $j$-th variable
where $\mathtt{s_j}$ denotes the signed-ness of the variable, 
$\mathtt{iwl_j}$ denotes the integer wordlength and $\mathtt{fwl_j}$ denotes
the fraction wordlength.
%$fi$ function constructs a fixed-point datatype
%in Matlab for the given sign-bit, wordlength and fractional
%wordlength.
\begin{algorithm}
\caption{Fixed-point program to compute area of circle}
\label{icse12:proc:ch1:fxcircle}
\begin{algorithmic}[style=tt]
\REQUIRE $\mathtt{radius}$, 
$\mathtt{\langle s_j,iwl_j,fwl_j \rangle}$ for $\mathtt{j=1,2,3,4}$
\ENSURE $\mathtt{area}$
\STATE $\mathbf{fx \langle s_1,iwl_1,fwl_1 \rangle}$ $\mathtt{mypi}$
\STATE $\mathbf{fx \langle s_2,iwl_2,fwl_2 \rangle}$ $\mathtt{radius}$
\STATE $\mathbf{fx \langle s_3,iwl_3,fwl_3 \rangle}$ $\mathtt{t}$
\STATE $\mathbf{fx \langle s_4,iwl_4,fwl_4 \rangle}$ $\mathtt{area}$
\STATE $\mathtt{mypi=3.14159265358979323846}$ 
\STATE $\mathtt{t=radius \times radius}$  
\STATE $\mathtt{area=mypi \times t}$
\RETURN $\mathtt{area}$
\end{algorithmic}
\end{algorithm}

We use $F_{fl}(X)$ to 
denote the floating-point program with inputs $X = x_1,x_2,\ldots,x_n$
and  $F_{fx}(X,\fxtype)$ to denote the fixed-point version of the program with
fixed-point type $\fxtype$.


\subsection{Input Domain}

The context in which a numerical fixed-point program 
$F_{fx}(X,\fxtype)$ is executed
often provides a precondition that must be satisfied
by valid inputs $(x_1,x_2,\ldots,x_n)$. This defines the input domain 
denoted by  $Dom(X)$.\\
\\
\noindent \textbf{Example 4.2:} In our example of computing area of a circle,
our interest is in radius in the interval $[0.1,2]$
and so the input domain $Dom(\mathtt{radius})$ 
is $$\mathtt{radius} \geq 0.1 \wedge \mathtt{radius} < 2$$

\subsection{Correctness Condition for Accuracy}

Correctness condition for accuracy involves specification
of a suitable error function and a maximum threshold of
error that the fixed-point program can have with respect to 
floating-point program. Let $F_{fl}(X)$ be floating-point
and  
$F_{fx}(X,\fxtype)$  be the corresponding fixed-point function
with fixed-point type $\fxtype$.
The error function $Err(F_{fl}(X),F_{fx}(X,\fxtype))$ 
is provided by the user
along with the maximum error threshold $\maxErr$.
Some common error functions can be:
\begin{itemize}
\item Absolute difference between the floating-point function
and fixed-point function, that is, $$\left |F_{fl}(X) - F_{fx}(X,\fxtype) \right|$$.
\item Relative difference between the floating-point function 
and fixed-point function, that is, $$\left |\frac{F_{fl}(X) - F_{fx}(X,\fxtype)}{F_{fl}(X)} \right|$$.
\item Moderated relative difference, that is, $$\left |\frac{F_{fl}(X) - F_{fx}(X,\fxtype)}{F_{fl}(X)+ \delta} \right|$$ which approaches relative difference
for $F_{fl}(X)>> \delta$ and approaches weighted absolute difference for $F_{fl}(X) << \delta$. When $F_{fl}(X)$ can be zero
for some values of $X$, the moderated relative difference remains bounded unlike
the relative difference which becomes unbounded.

\end{itemize}

%Any error function (linear or nonlinear) can be used since
%our technique evaluates the error on a given input and thus,
%any computable function is acceptable as an error function.
The {\em correctness condition for accuracy}
requires that for all inputs in the
provided {\em input domain} $Dom(X)$, the error function
$Err(F_{fl}(X),F_{fx}(X,\fxtype))$ is below 
the specified threshold $\maxErr$,
that is,
$$ \forall X \in Dom(X) \;. \;
Err(F_{fl}(X),F_{fx}(X,\fxtype)) \leq \maxErr$$


\noindent \textbf{Example 4.3:} In our running example of 
computing area of a circle, 
the error function is chosen to be relative difference, and the 
correctness condition for accuracy is
$$\forall \mathtt{radius}, \; such \; that, \;
\mathtt{radius} \geq 0.1 \wedge \mathtt{radius} < 2$$
$$\frac{F_{fl}(\mathtt{radius}) - F_{fx}(\mathtt{radius},\fxtype)}{F_{fl}(\mathtt{radius})}  \leq 0.1$$

\subsection{Implementation Cost Model}

The scaffold 
for the floating-point program is obtained from the fixed-point program.
The synthesis process discovers the fixed-point types of the variables
used in the program.
So, the cost of different possible implementations differs only 
in the fixed-point types of the variables.
Recall that fixed-point type is 
3-tuple  
$\mathtt{\langle s_j,iwl_j,fwl_j \rangle}$ for $j$-th variable
where $\mathtt{s_j}$ denotes the signed-ness of the variable, 
$\mathtt{iwl_j}$ denotes the integer wordlength and $\mathtt{fwl_j}$ denotes
the fraction wordlength.
The {\em cost model} of the implementation
is a function of the chosen fixed-point types of
the variables. In practice, it is often just a function 
of the total wordlengths ($\wl = \iwl + \fwl$) of the variables.
The cost model can incorporate
implementation area, power and other metrics of interest. 
For a given fixed-point program $F_{fx}(X,\fxtype)$,
let $T = \{t_1, t_2, \ldots, t_k\}$ be the set of 
fixed-point program variables with corresponding
types $\{\fxtype(t_1), \fxtype(t_2), \ldots, \fxtype(t_k)\}$. 
The cost of the fixed-point implementation 
is a function from
the fixed-point types of the variables to
a real value, that is,
cost of the fixed-point program $F_{fx}$ is 
$$\fxcost: (\fxtype(t_1),\fxtype(t_2),\ldots,\fxtype(t_k)) \rightarrow \mathbb{R} $$
A number of area-cost and power-cost
models~\cite{chien-vlsi97,macii-iccad98,clarke-ISCAS06,constantinides-FCCM02}
of hardware implementing fixed-point program can be used as cost function
in our technique. \\
\\
\noindent \textbf{Example 4.4:} The area model proposed
by Constantinides et al~\cite{constantinides-FCCM02} 
for the running example yields the following cost function.
We use this cost model in all our examples.
$$\fxcost (\fxtype(\mathtt{mypi}),\fxtype(\mathtt{radius}),\fxtype(\mathtt{t}), \fxtype(\mathtt{area})) = $$
$$\fxcostdelay(\iwl(\mathtt{mypi}))$$ 
$$+ \fxcostmul(\iwl(\mathtt{radius}), \iwl(\mathtt{radius}), \iwl(\mathtt{t}))$$ 
$$+ \fxcostmul(\iwl(\mathtt{mypi}), \iwl(\mathtt{t}), \iwl(\mathtt{area}))$$
where $$\fxcostdelay(l) = l+1$$ and $$\fxcostmul(l_1,l_2,l) = 0.6 \times (l_1+1) * l_2 - 0.85 * (l_1 + l_2 - l)$$ .

Our technique can be used with any cost model. In all our experiments
as well as the running example,
we use the Constantinides model~\cite{constantinides-FCCM02}.

\subsection{Problem Definition}
\begin{definition}[Optimal Fixed-point Program Synthesis]
The optimal fixed-point program synthesis problem
is as follows. Given
\begin{enumerate}
\item  a floating-point program $F_{fx}(X,\fxtype(T))$ with fixed-point variables $T$,
\item  an input domain $Dom(X)$  
\item  a correctness condition $Err(F_{fl}(X),F_{fx}(X,\fxtype(T))) \leq \maxErr$
\item  a cost model $\fxcost(\fxtype(t_1),\fxtype(t_2),\ldots,\fxtype(t_k))$
\end{enumerate}
optimal fixed-point program synthesis problem is to discover
fixed-point types 
$$\fxtype(T)^* = \{ \fxtype(t_1), \fxtype(t_2), \ldots, \fxtype(t_k) \}$$
such that the fixed-point program $F_{fl}(X)$ with the above types for fixed-point
variables 
\begin{itemize}
\item (a) is correct with respect to the correctness condition for accuracy,
that is,
$$ \forall X \in Dom(X) \;.\; Err(F_{fl}(X),F_{fx}(X,\fxtype(T)^*)) \leq \maxErr$$
\item (b) has minimal
cost with respect to the given cost function among all fixed-point types
that satisfy condition (a), that is,
$$\fxtype(T)^* = \underset{\fxtype(T) \mathtt{\; satisfies \; (a)}}{\operatorname{argmin}} \; \fxcost(\fxtype(T))$$
\end{itemize}
\end{definition}
Our goal is to automated this 
search for fixed-point types in order 
to synthesize fixed-point program that is firstly, correct with respect to the
correctness condition for accuracy and then, optimal with respect to the
given cost model. We illustrate this problem using the running example
below.\\
\\
\noindent \textbf{Example 4.5: }
In our running example of computing the {\em area of a circle},
we need to discover $\fxtype(\mathtt{mypi}),$ $\fxtype(\mathtt{radius}),$ $\fxtype(\mathtt{t})$  
and $\fxtype(\mathtt{area})$
such that the fixed-point program  satisfies the correctness condition
$$(a) \;\; \forall \mathtt{radius},  \; such \; that, \;
\mathtt{radius} \geq 0.1 \wedge \mathtt{radius} < 2$$
$$\frac{F_{fl}(\mathtt{radius}) - F_{fx}(\mathtt{radius},\fxtype)}{F_{fl}(\mathtt{radius})}  \leq 0.1$$
and the cost is minimized, that is,
$$(b) \;\; \underset{\fxtype \mathtt{\; satisfies \; (a)}} {\operatorname{argmin}} \; \fxcost(\fxtype(\mathtt{mypi}, \mathtt{radius},\mathtt{t}, \mathtt{area}))$$
%\end{example}
We use this example to illustrate the trade-off between cost and error
and how, a human would use trial and error to discover the correct
wordlengths.


\begin{figure}[ht]
\includegraphics[width=3.5in]{circle1}
\caption{Wordlength 8}
\label{icse12:fig:circlearea8}
\end{figure}


\begin{figure}[ht]
\includegraphics[width=3.5in]{circle2}
\caption{Wordlength 12}
\label{icse12:fig:circlearea12}
\end{figure}


\begin{figure}[ht]
\includegraphics[width=3.5in]{circle3}
\caption{Wordlength 16}
\label{icse12:fig:circlearea16}
\end{figure}

 
\textbf{Case 1}: In the first
case, all wordlengths ($\wl$) are fixed to $8$. Integer wordlengths ($\iwl$)
are selected to avoid overflow and the remaining bits are used for fractional
wordlength ($\fwl$). Since all variables will always take positive values,
we set the signed-ness bit to $0$.
Thus, the fixed-point types for the variables are:
$\fxtype(\mathtt{mypi}) = \langle 0, 2, 6\rangle,
\fxtype(\mathtt{radius}) = \langle 0,1, 7\rangle,
\fxtype(\mathtt{t}) = \langle 0, 2, 6\rangle,
\fxtype(\mathtt{area}) = \langle 0, 4,4 \rangle$
The cost of the implementation is $81.80$ . 
Figure~\ref{icse12:fig:circlearea8}
illustrates both the relative and absolute difference between
the fixed-point and floating-point program with this wordlength. 
It is obtained by simulating all radius in the given domain at
intervals of $0.0001$. The horizontal line in the plots of 
relative error shows the maximum threshold of $0.01$.


\textbf{Case 2:} 
Increasing the wordlengths of all the fixed-point variables to $12$, 
increases the cost of implementation
to $179.80$.
The new fixed-point types for the variables are:
$\fxtype(\mathtt{mypi}) = \langle 0, 2, 10\rangle,
\fxtype(\mathtt{radius}) = \langle 0,1, 11\rangle,
\fxtype(\mathtt{t}) = \langle 0, 2, 10\rangle,
\fxtype(\mathtt{area}) = \langle 0, 4,8 \rangle$
but the relative and absolute difference between the fixed-point
and floating-point program is reduced as illustrated in 
Figure~\ref{icse12:fig:circlearea12}.
The correctness condition for accuracy is still not satisfied.


\textbf{Case 3}: 
Further increasing the wordlength to $16$ decreases the error to satisfy
the correctness criteria as illustrated in 
Figure~\ref{icse12:fig:circlearea16} but the cost of implementation rises to 
$316.20$. The fixed-point types for the variables are:
$\fxtype(\mathtt{mypi}) = \langle 0, 2, 6\rangle,$
 $\fxtype(\mathtt{radius}) = \langle 0, 1, 7\rangle,$
 $\fxtype(\mathtt{t}) = \langle 0, 2, 6\rangle,$
 $\fxtype(\mathtt{area}) = \langle 0, 4, 4 \rangle$.


Manual synthesis of fixed-point program would require
the developer to try simulations of this program with varying 
fixed-point types for 
different variables and identify the cases where 
the correctness condition is satisfied. The next step would
be to find the fixed-point type that minimizes the cost from among
all the types that satisfy the correctness condition.
Such a manual trial and error process is time-consuming and 
error prone. Another dimension of the problem is finding the set
of inputs for which the program needs to be simulated to check for the
correctness condition. Since the input domain can be very large,
it is not possible to simulate the program for all possible inputs.
Intelligent choice of the inputs to use in simulating 
the program is important for 
a practical synthesis approach. In the following
section, we present an automated approach to solve this problem.





==> probdef.tex <==

\section{Problem Definition} \label{icse12:sec:probdef}

Numerical computation with specified accuracy is of fundamental
importance in many applications such as digital signal processing and
control systems. Algorithms for these applications are often designed 
ignoring the finite precision of computer arithmetic. Quantization
errors due to finite precision are analyzed later. Floating-point
environments are very useful in providing a convenient design
and validation environment to designers who can use it to explore
the algorithm space and also quickly simulate the design using
standard floating-point units available on computers. When these algorithms
need to be implemented on hardware,  floating-point data types
are converted to fixed-point data types in order to reduce the cost
of hardware needed as well as to decrease the power requirement
and increase the speed of computation. 
The conversion from floating-point
to fixed-point often results into decreased computation
accuracy. An optimal selection of word-lengths
of fixed-point variables to ensure accuracy remains above the 
specified threshold and the implementation cost is low, 
is a challenging task.

Along with a floating-point implementation of numerical
computation, the user can provide additional specification
regarding the desired fixed-point implementation.
The floating-point program takes inputs from a given {\em input domain}.
This input domain can be provided as a logical condition on the
inputs.
Numerical computation is expected to have some
{\em specified threshold of numerical accuracy}
which can be provided as a correctness condition for the fixed-point
program.
Further, the fixed-point implementation has a cost associated
with it and an optimal implementation is
expected to take minimal cost. 
The user can provide a cost model for the implementation.
We use a simple illustrative example to explain the
problem of synthesizing optimal fixed-point program
from floating-point program, and then present the formal
problem definition.

\subsection{Floating-point Implementation}
Floating-point implementation of the numerical
computation provides the scaffold of the
fixed-point program. Each floating-point variable
needs to be translated to fixed-point datatype.
 and hence,
the synthesis task is that of discovering the 
appropriate wordlength of the fixed-point variables
such that the correctness criteria is met for all
inputs satisfying the input condition and the
implementation cost is minimized.\\
\\
\noindent \textbf{Example 4.1:} 
%\begin{example}
We present an example in Procedure~\ref{icse12:proc:ch1:fpcircle}
that illustrates this problem and the
difficulty that programmers face in doing the floating-point to 
fixed-point translation manually. The floating-point
program in this example takes $\mathtt{radius}$ as the input, and
computes the $\mathtt{area}$ of the circle with this $\mathtt{radius}$.

\begin{algorithm}
\caption{Floating-point program to compute area of circle}
\label{icse12:proc:ch1:fpcircle}
\begin{algorithmic} [style=tt]
\REQUIRE $\mathtt{radius}$
\ENSURE $\mathtt{area}$
\STATE \textbf {double} $\mathtt{mypi, radius, t, area}$
\STATE $\mathtt{mypi=3.14159265358979323846}$ 
\STATE $\mathtt{t=radius \times radius}$  
\STATE $\mathtt{area=mypi \times t}$
\RETURN $\mathtt{area}$
\end{algorithmic}
\end{algorithm}


From the provided floating-point program, it is
easy to extract the scaffold of the fixed-point
program. The only unknowns are the
fixed-point type of the variables $\mathtt{mypi, radius, t}$
and $\mathtt{area}$. So, the scaffold fixed-point
program takes as input both the radius and the wordlengths
for the fixed-point variables. 
Recall that the fixed-point
type is a 3-tuple  
$\mathtt{\langle s_j,iwl_j,fwl_j \rangle}$ for $j$-th variable
where $\mathtt{s_j}$ denotes the signed-ness of the variable, 
$\mathtt{iwl_j}$ denotes the integer wordlength and $\mathtt{fwl_j}$ denotes
the fraction wordlength.
%$fi$ function constructs a fixed-point datatype
%in Matlab for the given sign-bit, wordlength and fractional
%wordlength.
\begin{algorithm}
\caption{Fixed-point program to compute area of circle}
\label{icse12:proc:ch1:fxcircle}
\begin{algorithmic}[style=tt]
\REQUIRE $\mathtt{radius}$, 
$\mathtt{\langle s_j,iwl_j,fwl_j \rangle}$ for $\mathtt{j=1,2,3,4}$
\ENSURE $\mathtt{area}$
\STATE $\mathbf{fx \langle s_1,iwl_1,fwl_1 \rangle}$ $\mathtt{mypi}$
\STATE $\mathbf{fx \langle s_2,iwl_2,fwl_2 \rangle}$ $\mathtt{radius}$
\STATE $\mathbf{fx \langle s_3,iwl_3,fwl_3 \rangle}$ $\mathtt{t}$
\STATE $\mathbf{fx \langle s_4,iwl_4,fwl_4 \rangle}$ $\mathtt{area}$
\STATE $\mathtt{mypi=3.14159265358979323846}$ 
\STATE $\mathtt{t=radius \times radius}$  
\STATE $\mathtt{area=mypi \times t}$
\RETURN $\mathtt{area}$
\end{algorithmic}
\end{algorithm}

We use $F_{fl}(X)$ to 
denote the floating-point program with inputs $X = x_1,x_2,\ldots,x_n$
and  $F_{fx}(X,\fxtype)$ to denote the fixed-point version of the program with
fixed-point type $\fxtype$.


\subsection{Input Domain}

The context in which a numerical fixed-point program 
$F_{fx}(X,\fxtype)$ is executed
often provides a precondition that must be satisfied
by valid inputs $(x_1,x_2,\ldots,x_n)$. This defines the input domain 
denoted by  $Dom(X)$.\\
\\
\noindent \textbf{Example 4.2:} In our example of computing area of a circle,
our interest is in radius in the interval $[0.1,2]$
and so the input domain $Dom(\mathtt{radius})$ 
is $$\mathtt{radius} \geq 0.1 \wedge \mathtt{radius} < 2$$

\subsection{Correctness Condition for Accuracy}

Correctness condition for accuracy involves specification
of a suitable error function and a maximum threshold of
error that the fixed-point program can have with respect to 
floating-point program. Let $F_{fl}(X)$ be floating-point
and  
$F_{fx}(X,\fxtype)$  be the corresponding fixed-point function
with fixed-point type $\fxtype$.
The error function $Err(F_{fl}(X),F_{fx}(X,\fxtype))$ 
is provided by the user
along with the maximum error threshold $\maxErr$.
Some common error functions can be:
\begin{itemize}
\item Absolute difference between the floating-point function
and fixed-point function, that is, $$\left |F_{fl}(X) - F_{fx}(X,\fxtype) \right|$$.
\item Relative difference between the floating-point function 
and fixed-point function, that is, $$\left |\frac{F_{fl}(X) - F_{fx}(X,\fxtype)}{F_{fl}(X)} \right|$$.
\item Moderated relative difference, that is, $$\left |\frac{F_{fl}(X) - F_{fx}(X,\fxtype)}{F_{fl}(X)+ \delta} \right|$$ which approaches relative difference
for $F_{fl}(X)>> \delta$ and approaches weighted absolute difference for $F_{fl}(X) << \delta$. When $F_{fl}(X)$ can be zero
for some values of $X$, the moderated relative difference remains bounded unlike
the relative difference which becomes unbounded.

\end{itemize}

%Any error function (linear or nonlinear) can be used since
%our technique evaluates the error on a given input and thus,
%any computable function is acceptable as an error function.
The {\em correctness condition for accuracy}
requires that for all inputs in the
provided {\em input domain} $Dom(X)$, the error function
$Err(F_{fl}(X),F_{fx}(X,\fxtype))$ is below 
the specified threshold $\maxErr$,
that is,
$$ \forall X \in Dom(X) \;. \;
Err(F_{fl}(X),F_{fx}(X,\fxtype)) \leq \maxErr$$


\noindent \textbf{Example 4.3:} In our running example of 
computing area of a circle, 
the error function is chosen to be relative difference, and the 
correctness condition for accuracy is
$$\forall \mathtt{radius}, \; such \; that, \;
\mathtt{radius} \geq 0.1 \wedge \mathtt{radius} < 2$$
$$\frac{F_{fl}(\mathtt{radius}) - F_{fx}(\mathtt{radius},\fxtype)}{F_{fl}(\mathtt{radius})}  \leq 0.1$$

\subsection{Implementation Cost Model}

The scaffold 
for the floating-point program is obtained from the fixed-point program.
The synthesis process discovers the fixed-point types of the variables
used in the program.
So, the cost of different possible implementations differs only 
in the fixed-point types of the variables.
Recall that fixed-point type is 
3-tuple  
$\mathtt{\langle s_j,iwl_j,fwl_j \rangle}$ for $j$-th variable
where $\mathtt{s_j}$ denotes the signed-ness of the variable, 
$\mathtt{iwl_j}$ denotes the integer wordlength and $\mathtt{fwl_j}$ denotes
the fraction wordlength.
The {\em cost model} of the implementation
is a function of the chosen fixed-point types of
the variables. In practice, it is often just a function 
of the total wordlengths ($\wl = \iwl + \fwl$) of the variables.
The cost model can incorporate
implementation area, power and other metrics of interest. 
For a given fixed-point program $F_{fx}(X,\fxtype)$,
let $T = \{t_1, t_2, \ldots, t_k\}$ be the set of 
fixed-point program variables with corresponding
types $\{\fxtype(t_1), \fxtype(t_2), \ldots, \fxtype(t_k)\}$. 
The cost of the fixed-point implementation 
is a function from
the fixed-point types of the variables to
a real value, that is,
cost of the fixed-point program $F_{fx}$ is 
$$\fxcost: (\fxtype(t_1),\fxtype(t_2),\ldots,\fxtype(t_k)) \rightarrow \mathbb{R} $$
A number of area-cost and power-cost
models~\cite{chien-vlsi97,macii-iccad98,clarke-ISCAS06,constantinides-FCCM02}
of hardware implementing fixed-point program can be used as cost function
in our technique. \\
\\
\noindent \textbf{Example 4.4:} The area model proposed
by Constantinides et al~\cite{constantinides-FCCM02} 
for the running example yields the following cost function.
We use this cost model in all our examples.
$$\fxcost (\fxtype(\mathtt{mypi}),\fxtype(\mathtt{radius}),\fxtype(\mathtt{t}), \fxtype(\mathtt{area})) = $$
$$\fxcostdelay(\iwl(\mathtt{mypi}))$$ 
$$+ \fxcostmul(\iwl(\mathtt{radius}), \iwl(\mathtt{radius}), \iwl(\mathtt{t}))$$ 
$$+ \fxcostmul(\iwl(\mathtt{mypi}), \iwl(\mathtt{t}), \iwl(\mathtt{area}))$$
where $$\fxcostdelay(l) = l+1$$ and $$\fxcostmul(l_1,l_2,l) = 0.6 \times (l_1+1) * l_2 - 0.85 * (l_1 + l_2 - l)$$ .

Our technique can be used with any cost model. In all our experiments
as well as the running example,
we use the Constantinides model~\cite{constantinides-FCCM02}.

\subsection{Problem Definition}
\begin{definition}[Optimal Fixed-point Program Synthesis]
The optimal fixed-point program synthesis problem
is as follows. Given
\begin{enumerate}
\item  a floating-point program $F_{fx}(X,\fxtype(T))$ with fixed-point variables $T$,
\item  an input domain $Dom(X)$  
\item  a correctness condition $Err(F_{fl}(X),F_{fx}(X,\fxtype(T))) \leq \maxErr$
\item  a cost model $\fxcost(\fxtype(t_1),\fxtype(t_2),\ldots,\fxtype(t_k))$
\end{enumerate}
optimal fixed-point program synthesis problem is to discover
fixed-point types 
$$\fxtype(T)^* = \{ \fxtype(t_1), \fxtype(t_2), \ldots, \fxtype(t_k) \}$$
such that the fixed-point program $F_{fl}(X)$ with the above types for fixed-point
variables 
\begin{itemize}
\item (a) is correct with respect to the correctness condition for accuracy,
that is,
$$ \forall X \in Dom(X) \;.\; Err(F_{fl}(X),F_{fx}(X,\fxtype(T)^*)) \leq \maxErr$$
\item (b) has minimal
cost with respect to the given cost function among all fixed-point types
that satisfy condition (a), that is,
$$\fxtype(T)^* = \underset{\fxtype(T) \mathtt{\; satisfies \; (a)}}{\operatorname{argmin}} \; \fxcost(\fxtype(T))$$
\end{itemize}
\end{definition}
Our goal is to automated this 
search for fixed-point types in order 
to synthesize fixed-point program that is firstly, correct with respect to the
correctness condition for accuracy and then, optimal with respect to the
given cost model. We illustrate this problem using the running example
below.\\
\\
\noindent \textbf{Example 4.5: }
In our running example of computing the {\em area of a circle},
we need to discover $\fxtype(\mathtt{mypi}),$ $\fxtype(\mathtt{radius}),$ $\fxtype(\mathtt{t})$  
and $\fxtype(\mathtt{area})$
such that the fixed-point program  satisfies the correctness condition
$$(a) \;\; \forall \mathtt{radius},  \; such \; that, \;
\mathtt{radius} \geq 0.1 \wedge \mathtt{radius} < 2$$
$$\frac{F_{fl}(\mathtt{radius}) - F_{fx}(\mathtt{radius},\fxtype)}{F_{fl}(\mathtt{radius})}  \leq 0.1$$
and the cost is minimized, that is,
$$(b) \;\; \underset{\fxtype \mathtt{\; satisfies \; (a)}} {\operatorname{argmin}} \; \fxcost(\fxtype(\mathtt{mypi}, \mathtt{radius},\mathtt{t}, \mathtt{area}))$$
%\end{example}
We use this example to illustrate the trade-off between cost and error
and how, a human would use trial and error to discover the correct
wordlengths.


\begin{figure}[ht]
\includegraphics[width=6in]{circle1}
\caption{Wordlength 8}
\label{icse12:fig:circlearea8}
\end{figure}


\begin{figure}[ht]
\includegraphics[width=6in]{circle2}
\caption{Wordlength 12}
\label{icse12:fig:circlearea12}
\end{figure}


\begin{figure}[ht]
\includegraphics[width=6in]{circle3}
\caption{Wordlength 16}
\label{icse12:fig:circlearea16}
\end{figure}

 
\textbf{Case 1}: In the first
case, all wordlengths ($\wl$) are fixed to $8$. Integer wordlengths ($\iwl$)
are selected to avoid overflow and the remaining bits are used for fractional
wordlength ($\fwl$). Since all variables will always take positive values,
we set the signed-ness bit to $0$.
Thus, the fixed-point types for the variables are:
$\fxtype(\mathtt{mypi}) = \langle 0, 2, 6\rangle,
\fxtype(\mathtt{radius}) = \langle 0,1, 7\rangle,
\fxtype(\mathtt{t}) = \langle 0, 2, 6\rangle,
\fxtype(\mathtt{area}) = \langle 0, 4,4 \rangle$
The cost of the implementation is $81.80$ . 
Figure~\ref{icse12:fig:circlearea8}
illustrates both the relative and absolute difference between
the fixed-point and floating-point program with this wordlength. 
It is obtained by simulating all radius in the given domain at
intervals of $0.0001$. The horizontal line in the plots of 
relative error shows the maximum threshold of $0.01$.


\textbf{Case 2:} 
Increasing the wordlengths of all the fixed-point variables to $12$, 
increases the cost of implementation
to $179.80$.
The new fixed-point types for the variables are:
$\fxtype(\mathtt{mypi}) = \langle 0, 2, 10\rangle,
\fxtype(\mathtt{radius}) = \langle 0,1, 11\rangle,
\fxtype(\mathtt{t}) = \langle 0, 2, 10\rangle,
\fxtype(\mathtt{area}) = \langle 0, 4,8 \rangle$
but the relative and absolute difference between the fixed-point
and floating-point program is reduced as illustrated in 
Figure~\ref{icse12:fig:circlearea12}.
The correctness condition for accuracy is still not satisfied.


\textbf{Case 3}: 
Further increasing the wordlength to $16$ decreases the error to satisfy
the correctness criteria as illustrated in 
Figure~\ref{icse12:fig:circlearea16} but the cost of implementation rises to 
$316.20$. The fixed-point types for the variables are:
$\fxtype(\mathtt{mypi}) = \langle 0, 2, 6\rangle,$
 $\fxtype(\mathtt{radius}) = \langle 0, 1, 7\rangle,$
 $\fxtype(\mathtt{t}) = \langle 0, 2, 6\rangle,$
 $\fxtype(\mathtt{area}) = \langle 0, 4, 4 \rangle$.


Manual synthesis of fixed-point program would require
the developer to try simulations of this program with varying 
fixed-point types for 
different variables and identify the cases where 
the correctness condition is satisfied. The next step would
be to find the fixed-point type that minimizes the cost from among
all the types that satisfy the correctness condition.
Such a manual trial and error process is time-consuming and 
error prone. Another dimension of the problem is finding the set
of inputs for which the program needs to be simulated to check for the
correctness condition. Since the input domain can be very large,
it is not possible to simulate the program for all possible inputs.
Intelligent choice of the inputs to use in simulating 
the program is important for 
a practical synthesis approach. In the following
section, we present an automated approach to solve this problem.





==> sig-alternate.cls.1 <==
% SIG-ALTERNATE.CLS - VERSION 2.4
% "COMPATIBLE" WITH THE "ACM_PROC_ARTICLE-SP.CLS" V3.2SP
% Gerald Murray - April 22nd. 2009
%
% ---- Start of 'updates'  ----
%
% Changed $5 fee to $10 - Gerry
% April 22nd. 2009 - Fixed 'Natbib' incompatibility problem - Gerry
% April 22nd. 2009 - Fixed 'Babel' incompatibility problem - Gerry
% April 22nd. 2009 - Inserted various bug-fixes and improvements - Gerry
%
% To produce Type 1 fonts in the document plus allow for 'normal LaTeX accenting' in the critical areas;
% title, author block, section-heads, confname, etc. etc. 
% i.e. the whole purpose of this version update is to NOT resort to 'inelegant accent patches'.
% After much research, three extra .sty packages were added to the the tail (ae, aecompl, aeguill) to solve,
% in particular, the accenting problem(s). We _could_ ask authors (via instructions/sample file) to 'include' these in
% the source .tex file - in the preamble - but if everything is already provided ('behind the scenes' - embedded IN the .cls)
% then this is less work for authors and also makes everything appear 'vanilla'.
% NOTE: all 'patchwork accenting" has been commented out (here) and is no longer 'used' in the sample .tex file (either).
% Gerry June 2007
%
% Patch for accenting in conference name/location. Gerry May 3rd. 2007
% Rule widths changed to .5, author count (>6) fixed, roll-back for Type 3 problem. Gerry March 20th. 2007
% Changes made to 'modernize' the fontnames but esp. for MikTeX users V2.4/2.5 - Nov. 30th. 2006
% Updated the \email definition to allow for its use inside of 'shared affiliations' - Nov. 30th. 2006
% Fixed the 'section number depth value' - Nov. 30th. 2006
%
% Footnotes inside table cells using \minipage (Oct. 2002)
% Georgia fixed bug in sub-sub-section numbering in paragraphs (July 29th. 2002)
% JS/GM fix to vertical spacing before Proofs (July 30th. 2002)
%
% Made the Permission Statement / Conference Info / Copyright Info
% 'user definable' in the source .tex file OR automatic if
% not specified.
%
% Allowance made to switch default fonts between those systems using
% normal/modern font names and those using 'Type 1' or 'Truetype' fonts.
% See LINE NUMBER 255 for details.
% Also provided for enumerated/annotated Corollaries 'surrounded' by
% enumerated Theorems (line 848).
% Gerry November 11th. 1999
%
% ---- End of 'updates' ----
%
\def\fileversion{v2.4}          % for ACM's tracking purposes
\def\filedate{April 22, 2009}    % Gerry Murray's tracking data
\def\docdate {Wednesday 22nd. April 2009} % Gerry Murray (with deltas to doc}
\usepackage{epsfig}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
% Need this for accents in Arial/Helvetica
%\usepackage[T1]{fontenc}  % Gerry March 12, 2007 - causes Type 3 problems (body text)
%\usepackage{textcomp}
%
% SIG-ALTERNATE DOCUMENT STYLE
% G.K.M. Tobin August-October 1999
%    adapted from ARTICLE document style by Ken Traub, Olin Shivers
%    also using elements of esub2acm.cls
% HEAVILY MODIFIED, SUBSEQUENTLY, BY GERRY MURRAY 2000
% ARTICLE DOCUMENT STYLE -- Released 16 March 1988
%    for LaTeX version 2.09
% Copyright (C) 1988 by Leslie Lamport
%
%
%%% sig-alternate.cls is an 'ALTERNATE' document style for producing
%%% two-column camera-ready pages for ACM conferences.
%%% THIS FILE DOES NOT STRICTLY ADHERE TO THE SIGS (BOARD-ENDORSED)
%%% PROCEEDINGS STYLE. It has been designed to produce a 'tighter'
%%% paper in response to concerns over page budgets.
%%% The main features of this style are:
%%%
%%% 1)  Two columns.
%%% 2)  Side and top margins of 4.5pc, bottom margin of 6pc, column gutter of
%%%     2pc, hence columns are 20pc wide and 55.5pc tall.  (6pc =3D 1in, approx)
%%% 3)  First page has title information, and an extra 6pc of space at the
%%%     bottom of the first column for the ACM copyright notice.
%%% 4)  Text is 9pt on 10pt baselines; titles (except main) are 9pt bold.
%%%
%%%
%%% There are a few restrictions you must observe:
%%%
%%% 1)  You cannot change the font size; ACM wants you to use 9pt.
%%% 3)  You must start your paper with the \maketitle command.  Prior to the
%%%     \maketitle you must have \title and \author commands.  If you have a
%%%     \date command it will be ignored; no date appears on the paper, since
%%%     the proceedings will have a date on the front cover.
%%% 4)  Marginal paragraphs, tables of contents, lists of figures and tables,
%%%     and page headings are all forbidden.
%%% 5)  The `figure' environment will produce a figure one column wide; if you
%%%     want one that is two columns wide, use `figure*'.
%%%
%
%%% Copyright Space:
%%% This style automatically reserves 1" blank space at the bottom of page 1/
%%% column 1.  This space can optionally be filled with some text using the
%%% \toappear{...} command.  If used, this command must be BEFORE the \maketitle
%%% command.  If this command is defined AND [preprint] is on, then the
%%% space is filled with the {...} text (at the bottom); otherwise, it is
%%% blank.  If you use \toappearbox{...} instead of \toappear{...} then a
%%% box will be drawn around the text (if [preprint] is on).
%%%
%%% A typical usage looks like this:
%%%     \toappear{To appear in the Ninth AES Conference on Medievil Lithuanian
%%%               Embalming Technique, June 1991, Alfaretta, Georgia.}
%%% This will be included in the preprint, and left out of the conference
%%% version.
%%%
%%% WARNING:
%%% Some dvi-ps converters heuristically allow chars to drift from their
%%% true positions a few pixels. This may be noticeable with the 9pt sans-serif
%%% bold font used for section headers.
%%% You may turn this hackery off via the -e option:
%%%     dvips -e 0 foo.dvi >foo.ps
%%%
\typeout{Document Class 'sig-alternate' <22nd. April '09>.  Modified by G.K.M. Tobin/Gerry Murray}
\typeout{Based in part upon document Style `acmconf' <22 May 89>. Hacked 4/91 by}
\typeout{shivers@cs.cmu.edu, 4/93 by theobald@cs.mcgill.ca}
\typeout{Excerpts were taken from (Journal Style) 'esub2acm.cls'.}
\typeout{****** Bugs/comments/suggestions/technicalities to Gerry Murray -- murray@hq.acm.org ******}
\typeout{Questions on the style, SIGS policies, etc. to Adrienne Griscti griscti@acm.org}
\oddsidemargin 4.5pc
\evensidemargin 4.5pc
\advance\oddsidemargin by -1in  % Correct for LaTeX gratuitousness
\advance\evensidemargin by -1in % Correct for LaTeX gratuitousness
\marginparwidth 0pt             % Margin pars are not allowed.
\marginparsep 11pt              % Horizontal space between outer margin and
                                % marginal note

                                % Top of page:
\topmargin 4.5pc                % Nominal distance from top of page to top of
                                % box containing running head.
\advance\topmargin by -1in      % Correct for LaTeX gratuitousness
\headheight 0pt                 % Height of box containing running head.
\headsep 0pt                    % Space between running head and text.
                                % Bottom of page:
\footskip 30pt                  % Distance from baseline of box containing foot
                                % to baseline of last line of text.
\@ifundefined{footheight}{\newdimen\footheight}{}% this is for LaTeX2e
\footheight 12pt                % Height of box containing running foot.

%% Must redefine the top margin so there's room for headers and
%% page numbers if you are using the preprint option. Footers
%% are OK as is. Olin.
\advance\topmargin by -37pt     % Leave 37pt above text for headers
\headheight 12pt                % Height of box containing running head.
\headsep 25pt                   % Space between running head and text.

\textheight 666pt       % 9 1/4 column height
\textwidth 42pc         % Width of text line.
                        % For two-column mode:
\columnsep 2pc          %    Space between columns
\columnseprule 0pt      %    Width of rule between columns.
\hfuzz 1pt              % Allow some variation in column width, otherwise it's
                        % too hard to typeset in narrow columns.

\footnotesep 5.6pt      % Height of strut placed at the beginning of every
                        % footnote =3D height of normal \footnotesize strut,
                        % so no extra space between footnotes.

\skip\footins 8.1pt plus 4pt minus 2pt  % Space between last line of text and
                                        % top of first footnote.
\floatsep 11pt plus 2pt minus 2pt       % Space between adjacent floats moved
                                        % to top or bottom of text page.
\textfloatsep 18pt plus 2pt minus 4pt   % Space between main text and floats
                                        % at top or bottom of page.
\intextsep 11pt plus 2pt minus 2pt      % Space between in-text figures and
                                        % text.
\@ifundefined{@maxsep}{\newdimen\@maxsep}{}% this is for LaTeX2e
\@maxsep 18pt                           % The maximum of \floatsep,
                                        % \textfloatsep and \intextsep (minus
                                        % the stretch and shrink).
\dblfloatsep 11pt plus 2pt minus 2pt    % Same as \floatsep for double-column
                                        % figures in two-column mode.
\dbltextfloatsep 18pt plus 2pt minus 4pt% \textfloatsep for double-column
                                        % floats.
\@ifundefined{@dblmaxsep}{\newdimen\@dblmaxsep}{}% this is for LaTeX2e
\@dblmaxsep 18pt                        % The maximum of \dblfloatsep and
                                        % \dbltexfloatsep.
\@fptop 0pt plus 1fil    % Stretch at top of float page/column. (Must be
                         % 0pt plus ...)
\@fpsep 8pt plus 2fil    % Space between floats on float page/column.
\@fpbot 0pt plus 1fil    % Stretch at bottom of float page/column. (Must be
                         % 0pt plus ... )
\@dblfptop 0pt plus 1fil % Stretch at top of float page. (Must be 0pt plus ...)
\@dblfpsep 8pt plus 2fil % Space between floats on float page.
\@dblfpbot 0pt plus 1fil % Stretch at bottom of float page. (Must be
                         % 0pt plus ... )
\marginparpush 5pt       % Minimum vertical separation between two marginal
                         % notes.

\parskip 0pt plus 1pt            % Extra vertical space between paragraphs.
\parindent 9pt  % GM July 2000 / was 0pt - width of paragraph indentation.
\partopsep 2pt plus 1pt minus 1pt% Extra vertical space, in addition to
                                 % \parskip and \topsep, added when user
                                 % leaves blank line before environment.

\@lowpenalty   51       % Produced by \nopagebreak[1] or \nolinebreak[1]
\@medpenalty  151       % Produced by \nopagebreak[2] or \nolinebreak[2]
\@highpenalty 301       % Produced by \nopagebreak[3] or \nolinebreak[3]

\@beginparpenalty -\@lowpenalty % Before a list or paragraph environment.
\@endparpenalty   -\@lowpenalty % After a list or paragraph environment.
\@itempenalty     -\@lowpenalty % Between list items.

%\@namedef{ds@10pt}{\@latexerr{The `10pt' option is not allowed in the `acmconf'
\@namedef{ds@10pt}{\ClassError{The `10pt' option is not allowed in the `acmconf'	% January 2008
  document style.}\@eha}
%\@namedef{ds@11pt}{\@latexerr{The `11pt' option is not allowed in the `acmconf'
\@namedef{ds@11pt}{\ClassError{The `11pt' option is not allowed in the `acmconf'	% January 2008
  document style.}\@eha}
%\@namedef{ds@12pt}{\@latexerr{The `12pt' option is not allowed in the `acmconf'
\@namedef{ds@12pt}{\ClassError{The `12pt' option is not allowed in the `acmconf'	% January 2008
  document style.}\@eha}

\@options

\lineskip 2pt           % \lineskip is 1pt for all font sizes.
\normallineskip 2pt
\def\baselinestretch{1}

\abovedisplayskip 9pt plus2pt minus4.5pt%
\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip  \z@ plus3pt%
\belowdisplayshortskip  5.4pt plus3pt minus3pt%
\let\@listi\@listI     % Setting of \@listi added 9 Jun 87

\def\small{\@setsize\small{9pt}\viiipt\@viiipt
\abovedisplayskip 7.6pt plus 3pt minus 4pt%
\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip \z@ plus2pt%
\belowdisplayshortskip 3.6pt plus2pt minus 2pt
\def\@listi{\leftmargin\leftmargini %% Added 22 Dec 87
\topsep 4pt plus 2pt minus 2pt\parsep 2pt plus 1pt minus 1pt
\itemsep \parsep}}

\def\footnotesize{\@setsize\footnotesize{9pt}\ixpt\@ixpt
\abovedisplayskip 6.4pt plus 2pt minus 4pt%
\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip \z@ plus 1pt%
\belowdisplayshortskip 2.7pt plus 1pt minus 2pt
\def\@listi{\leftmargin\leftmargini %% Added 22 Dec 87
\topsep 3pt plus 1pt minus 1pt\parsep 2pt plus 1pt minus 1pt
\itemsep \parsep}}

\newcount\aucount
\newcount\originalaucount
\newdimen\auwidth
\auwidth=\textwidth
\newdimen\auskip
\newcount\auskipcount
\newdimen\auskip
\global\auskip=1pc
\newdimen\allauboxes
\allauboxes=\auwidth
\newtoks\addauthors
\newcount\addauflag
\global\addauflag=0 %Haven't shown additional authors yet

\newtoks\subtitletext
\gdef\subtitle#1{\subtitletext={#1}}

\gdef\additionalauthors#1{\addauthors={#1}}

\gdef\numberofauthors#1{\global\aucount=#1
\ifnum\aucount>3\global\originalaucount=\aucount \global\aucount=3\fi %g}  % 3 OK - Gerry March 2007
\global\auskipcount=\aucount\global\advance\auskipcount by 1
\global\multiply\auskipcount by 2
\global\multiply\auskip by \auskipcount
\global\advance\auwidth by -\auskip
\global\divide\auwidth by \aucount}

% \and was modified to count the number of authors.  GKMT 12 Aug 1999
\def\alignauthor{%                  % \begin{tabular}
\end{tabular}%
  \begin{tabular}[t]{p{\auwidth}}\centering}%

%  *** NOTE *** NOTE *** NOTE *** NOTE ***
%  If you have 'font problems' then you may need
%  to change these, e.g. 'arialb' instead of "arialbd".
%  Gerry Murray 11/11/1999
%  *** OR ** comment out block A and activate block B or vice versa.
% **********************************************
%
%  -- Start of block A -- (Type 1 or Truetype fonts)
%\newfont{\secfnt}{timesbd at 12pt} % was timenrb originally - now is timesbd
%\newfont{\secit}{timesbi at 12pt}   %13 Jan 00 gkmt
%\newfont{\subsecfnt}{timesi at 11pt} % was timenrri originally - now is timesi
%\newfont{\subsecit}{timesbi at 11pt} % 13 Jan 00 gkmt -- was times changed to timesbi gm 2/4/2000
%                         % because "normal" is italic, "italic" is Roman
%\newfont{\ttlfnt}{arialbd at 18pt} % was arialb originally - now is arialbd
%\newfont{\ttlit}{arialbi at 18pt}    % 13 Jan 00 gkmt
%\newfont{\subttlfnt}{arial at 14pt} % was arialr originally - now is arial
%\newfont{\subttlit}{ariali at 14pt} % 13 Jan 00 gkmt
%\newfont{\subttlbf}{arialbd at 14pt}  % 13 Jan 00 gkmt
%\newfont{\aufnt}{arial at 12pt} % was arialr originally - now is arial
%\newfont{\auit}{ariali at 12pt} % 13 Jan 00 gkmt
%\newfont{\affaddr}{arial at 10pt} % was arialr originally - now is arial
%\newfont{\affaddrit}{ariali at 10pt} %13 Jan 00 gkmt
%\newfont{\eaddfnt}{arial at 12pt} % was arialr originally - now is arial
%\newfont{\ixpt}{times at 9pt} % was timenrr originally - now is times
%\newfont{\confname}{timesi at 8pt} % was timenrri - now is timesi
%\newfont{\crnotice}{times at 8pt} % was timenrr originally - now is times
%\newfont{\ninept}{times at 9pt} % was timenrr originally - now is times

% *********************************************
%  -- End of block A --
%
%
% -- Start of block B -- UPDATED FONT NAMES
% *********************************************
% Gerry Murray 11/30/2006
% *********************************************
\newfont{\secfnt}{ptmb8t at 12pt}
\newfont{\secit}{ptmbi8t at 12pt}    %13 Jan 00 gkmt
\newfont{\subsecfnt}{ptmri8t at 11pt}
\newfont{\subsecit}{ptmbi8t at 11pt}  % 
\newfont{\ttlfnt}{phvb8t at 18pt}
\newfont{\ttlit}{phvbo8t at 18pt}    % GM 2/4/2000
\newfont{\subttlfnt}{phvr8t at 14pt}
\newfont{\subttlit}{phvro8t at 14pt} % GM 2/4/2000
\newfont{\subttlbf}{phvb8t at 14pt}  % 13 Jan 00 gkmt
\newfont{\aufnt}{phvr8t at 12pt}
\newfont{\auit}{phvro8t at 12pt}     % GM 2/4/2000
\newfont{\affaddr}{phvr8t at 10pt}
\newfont{\affaddrit}{phvro8t at 10pt} % GM 2/4/2000
\newfont{\eaddfnt}{phvr8t at 12pt}
\newfont{\ixpt}{ptmr8t at 9pt}
\newfont{\confname}{ptmri8t at 8pt}
\newfont{\crnotice}{ptmr8t at 8pt}
\newfont{\ninept}{ptmr8t at 9pt}
% +++++++++++++++++++++++++++++++++++++++++++++
% -- End of block B --

%\def\email#1{{{\eaddfnt{\vskip 4pt#1}}}}
% If we have an email, inside a "shared affiliation" then we need the following instead
\def\email#1{{{\eaddfnt{\par #1}}}}       % revised  - GM - 11/30/2006

\def\addauthorsection{\ifnum\originalaucount>6  % was 3 - Gerry March 2007
    \section{Additional Authors}\the\addauthors
  \fi}

\newcount\savesection
\newcount\sectioncntr
\global\sectioncntr=1

\setcounter{secnumdepth}{3}

\def\appendix{\par
\section*{APPENDIX}
\setcounter{section}{0}
 \setcounter{subsection}{0}
 \def\thesection{\Alph{section}} }

\leftmargini 22.5pt
\leftmarginii 19.8pt    % > \labelsep + width of '(m)'
\leftmarginiii 16.8pt   % > \labelsep + width of 'vii.'
\leftmarginiv 15.3pt    % > \labelsep + width of 'M.'
\leftmarginv 9pt
\leftmarginvi 9pt

\leftmargin\leftmargini
\labelsep 4.5pt
\labelwidth\leftmargini\advance\labelwidth-\labelsep

\def\@listI{\leftmargin\leftmargini \parsep 3.6pt plus 2pt minus 1pt%
\topsep 7.2pt plus 2pt minus 4pt%
\itemsep 3.6pt plus 2pt minus 1pt}

\let\@listi\@listI
\@listi

\def\@listii{\leftmargin\leftmarginii
   \labelwidth\leftmarginii\advance\labelwidth-\labelsep
   \topsep 3.6pt plus 2pt minus 1pt
   \parsep 1.8pt plus 0.9pt minus 0.9pt
   \itemsep \parsep}

\def\@listiii{\leftmargin\leftmarginiii
    \labelwidth\leftmarginiii\advance\labelwidth-\labelsep
    \topsep 1.8pt plus 0.9pt minus 0.9pt
    \parsep \z@ \partopsep 1pt plus 0pt minus 1pt
    \itemsep \topsep}

\def\@listiv{\leftmargin\leftmarginiv
     \labelwidth\leftmarginiv\advance\labelwidth-\labelsep}

\def\@listv{\leftmargin\leftmarginv
     \labelwidth\leftmarginv\advance\labelwidth-\labelsep}

\def\@listvi{\leftmargin\leftmarginvi
     \labelwidth\leftmarginvi\advance\labelwidth-\labelsep}

\def\labelenumi{\theenumi.}
\def\theenumi{\arabic{enumi}}

\def\labelenumii{(\theenumii)}
\def\theenumii{\alph{enumii}}
\def\p@enumii{\theenumi}

\def\labelenumiii{\theenumiii.}
\def\theenumiii{\roman{enumiii}}
\def\p@enumiii{\theenumi(\theenumii)}

\def\labelenumiv{\theenumiv.}
\def\theenumiv{\Alph{enumiv}}
\def\p@enumiv{\p@enumiii\theenumiii}

\def\labelitemi{$\bullet$}
\def\labelitemii{\bf --}
\def\labelitemiii{$\ast$}
\def\labelitemiv{$\cdot$}

\def\verse{\let\\=\@centercr
  \list{}{\itemsep\z@ \itemindent -1.5em\listparindent \itemindent
          \rightmargin\leftmargin\advance\leftmargin 1.5em}\item[]}
\let\endverse\endlist

\def\quotation{\list{}{\listparindent 1.5em
    \itemindent\listparindent
    \rightmargin\leftmargin \parsep 0pt plus 1pt}\item[]}
\let\endquotation=\endlist

\def\quote{\list{}{\rightmargin\leftmargin}\item[]}
\let\endquote=\endlist

\def\descriptionlabel#1{\hspace\labelsep \bf #1}
\def\description{\list{}{\labelwidth\z@ \itemindent-\leftmargin
       \let\makelabel\descriptionlabel}}

\let\enddescription\endlist

\def\theequation{\arabic{equation}}

\arraycolsep 4.5pt   % Half the space between columns in an array environment.
\tabcolsep 5.4pt    % Half the space between columns in a tabular environment.
\arrayrulewidth .5pt % Width of rules in array and tabular environment. % (was .4) updated Gerry March 20 2007
\doublerulesep 1.8pt % Space between adjacent rules in array or tabular env.

\tabbingsep \labelsep   % Space used by the \' command.  (See LaTeX manual.)

\skip\@mpfootins =\skip\footins

\fboxsep =2.7pt      % Space left between box and text by \fbox and \framebox.
\fboxrule =.5pt      % Width of rules in box made by \fbox and \framebox. % (was .4) updated Gerry March 20 2007

\def\thepart{\Roman{part}} % Roman numeral part numbers.
\def\thesection       {\arabic{section}}
\def\thesubsection    {\thesection.\arabic{subsection}}
%\def\thesubsubsection {\thesubsection.\arabic{subsubsection}} % GM 7/30/2002
%\def\theparagraph     {\thesubsubsection.\arabic{paragraph}}  % GM 7/30/2002
\def\thesubparagraph  {\theparagraph.\arabic{subparagraph}}

\def\@pnumwidth{1.55em}
\def\@tocrmarg {2.55em}
\def\@dotsep{4.5}
\setcounter{tocdepth}{3}

%\def\tableofcontents{\@latexerr{\tableofcontents: Tables of contents are not
%  allowed in the `acmconf' document style.}\@eha}

\def\tableofcontents{\ClassError{%
    \string\tableofcontents\space is not allowed in the `acmconf' document	% January 2008
    style}\@eha}

\def\l@part#1#2{\addpenalty{\@secpenalty}
   \addvspace{2.25em plus 1pt}  % space above part line
   \begingroup
   \@tempdima 3em       % width of box holding part number, used by
     \parindent \z@ \rightskip \@pnumwidth      %% \numberline
     \parfillskip -\@pnumwidth
     {\large \bf        % set line in \large boldface
     \leavevmode        % TeX command to enter horizontal mode.
     #1\hfil \hbox to\@pnumwidth{\hss #2}}\par
     \nobreak           % Never break after part entry
   \endgroup}

\def\l@section#1#2{\addpenalty{\@secpenalty} % good place for page break
   \addvspace{1.0em plus 1pt}   % space above toc entry
   \@tempdima 1.5em             % width of box holding section number
   \begingroup
    \parindent  \z@ \rightskip \@pnumwidth
     \parfillskip -\@pnumwidth
     \bf                        % Boldface.
     \leavevmode                % TeX command to enter horizontal mode.
      \advance\leftskip\@tempdima %% added 5 Feb 88 to conform to
      \hskip -\leftskip           %% 25 Jan 88 change to \numberline
     #1\nobreak\hfil \nobreak\hbox to\@pnumwidth{\hss #2}\par
   \endgroup}


\def\l@subsection{\@dottedtocline{2}{1.5em}{2.3em}}
\def\l@subsubsection{\@dottedtocline{3}{3.8em}{3.2em}}
\def\l@paragraph{\@dottedtocline{4}{7.0em}{4.1em}}
\def\l@subparagraph{\@dottedtocline{5}{10em}{5em}}

%\def\listoffigures{\@latexerr{\listoffigures: Lists of figures are not
%  allowed in the `acmconf' document style.}\@eha}

\def\listoffigures{\ClassError{%
    \string\listoffigures\space is not allowed in the `acmconf' document	% January 2008
    style}\@eha}

\def\l@figure{\@dottedtocline{1}{1.5em}{2.3em}}

%\def\listoftables{\@latexerr{\listoftables: Lists of tables are not
%  allowed in the `acmconf' document style.}\@eha}
%\let\l@table\l@figure

\def\listoftables{\ClassError{%
    \string\listoftables\space is not allowed in the `acmconf' document		% January 2008
    style}\@eha}
 \let\l@table\l@figure

\def\footnoterule{\kern-3\p@
  \hrule width .5\columnwidth   % (was .4) updated Gerry March 20 2007
  \kern 2.6\p@}                 % The \hrule has default height of .4pt % (was .4) updated Gerry March 20 2007
% ------
\long\def\@makefntext#1{\noindent 
%\hbox to .5em{\hss$^{\@thefnmark}$}#1}   % original
\hbox to .5em{\hss\textsuperscript{\@thefnmark}}#1}  % C. Clifton / GM Oct. 2nd. 2002
% -------

\long\def\@maketntext#1{\noindent
#1}

\long\def\@maketitlenotetext#1#2{\noindent
            \hbox to 1.8em{\hss$^{#1}$}#2}

\setcounter{topnumber}{2}
\def\topfraction{.7}
\setcounter{bottomnumber}{1}
\def\bottomfraction{.3}
\setcounter{totalnumber}{3}
\def\textfraction{.2}
\def\floatpagefraction{.5}
\setcounter{dbltopnumber}{2}
\def\dbltopfraction{.7}
\def\dblfloatpagefraction{.5}

%
\long\def\@makecaption#1#2{
   \vskip \baselineskip
   \setbox\@tempboxa\hbox{\textbf{#1: #2}}
   \ifdim \wd\@tempboxa >\hsize % IF longer than one line:
       \textbf{#1: #2}\par               %   THEN set as ordinary paragraph.
     \else                      %   ELSE  center.
       \hbox to\hsize{\hfil\box\@tempboxa\hfil}\par
   \fi}

%

\long\def\@makecaption#1#2{
   \vskip 10pt
   \setbox\@tempboxa\hbox{\textbf{#1: #2}}
   \ifdim \wd\@tempboxa >\hsize % IF longer than one line:
       \textbf{#1: #2}\par                %   THEN set as ordinary paragraph.
     \else                      %   ELSE  center.
       \hbox to\hsize{\hfil\box\@tempboxa\hfil}
   \fi}

\@ifundefined{figure}{\newcounter {figure}} % this is for LaTeX2e

\def\fps@figure{tbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{Figure \thefigure}
\def\figure{\@float{figure}}
%\let\endfigure\end@float
\def\endfigure{\end@float} 		% Gerry January 2008
\@namedef{figure*}{\@dblfloat{figure}}
\@namedef{endfigure*}{\end@dblfloat}

\@ifundefined{table}{\newcounter {table}} % this is for LaTeX2e

\def\fps@table{tbp}
\def\ftype@table{2}
\def\ext@table{lot}
\def\fnum@table{Table \thetable}
\def\table{\@float{table}}
%\let\endtable\end@float
\def\endtable{\end@float}		% Gerry January 2008
\@namedef{table*}{\@dblfloat{table}}
\@namedef{endtable*}{\end@dblfloat}

\newtoks\titleboxnotes
\newcount\titleboxnoteflag

\def\maketitle{\par
 \begingroup
   \def\thefootnote{\fnsymbol{footnote}}
   \def\@makefnmark{\hbox
       to 0pt{$^{\@thefnmark}$\hss}}
     \twocolumn[\@maketitle]
\@thanks
 \endgroup
 \setcounter{footnote}{0}
 \let\maketitle\relax
 \let\@maketitle\relax
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\gdef\@subtitle{}\let\thanks\relax
 \@copyrightspace}

%% CHANGES ON NEXT LINES
\newif\if@ll % to record which version of LaTeX is in use

\expandafter\ifx\csname LaTeXe\endcsname\relax % LaTeX2.09 is used
\else% LaTeX2e is used, so set ll to true
\global\@lltrue
\fi

\if@ll
  \NeedsTeXFormat{LaTeX2e}
  \ProvidesClass{sig-alternate} [2009/04/22 - V2.4 - based on acmproc.cls V1.3 <Nov. 30 '99>]
  \RequirePackage{latexsym}% QUERY: are these two really needed?
  \let\dooptions\ProcessOptions
\else
  \let\dooptions\@options
\fi
%% END CHANGES

\def\@height{height}
\def\@width{width}
\def\@minus{minus}
\def\@plus{plus}
\def\hb@xt@{\hbox to}
\newif\if@faircopy
\@faircopyfalse
\def\ds@faircopy{\@faircopytrue}

\def\ds@preprint{\@faircopyfalse}

\@twosidetrue
\@mparswitchtrue
\def\ds@draft{\overfullrule 5\p@}
%% CHANGE ON NEXT LINE
\dooptions

\lineskip \p@
\normallineskip \p@
\def\baselinestretch{1}
\def\@ptsize{0} %needed for amssymbols.sty

%% CHANGES ON NEXT LINES
\if@ll% allow use of old-style font change commands in LaTeX2e
\@maxdepth\maxdepth
%
\DeclareOldFontCommand{\rm}{\ninept\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\DeclareRobustCommand*{\cal}{\@fontswitch{\relax}{\mathcal}}
\DeclareRobustCommand*{\mit}{\@fontswitch{\relax}{\mathnormal}}
\fi
%
\if@ll
 \renewcommand{\rmdefault}{cmr}  % was 'ttm'
% Note! I have also found 'mvr' to work ESPECIALLY well.
% Gerry - October 1999
% You may need to change your LV1times.fd file so that sc is
% mapped to cmcsc - -for smallcaps -- that is if you decide
% to change {cmr} to {times} above. (Not recommended)
  \renewcommand{\@ptsize}{}
  \renewcommand{\normalsize}{%
    \@setfontsize\normalsize\@ixpt{10.5\p@}%\ninept%
    \abovedisplayskip 6\p@ \@plus2\p@ \@minus\p@
    \belowdisplayskip \abovedisplayskip
    \abovedisplayshortskip 6\p@ \@minus 3\p@
    \belowdisplayshortskip 6\p@ \@minus 3\p@
    \let\@listi\@listI
  }
\else
  \def\@normalsize{%changed next to 9 from 10
    \@setsize\normalsize{9\p@}\ixpt\@ixpt
   \abovedisplayskip 6\p@ \@plus2\p@ \@minus\p@
    \belowdisplayskip \abovedisplayskip
    \abovedisplayshortskip 6\p@ \@minus 3\p@
    \belowdisplayshortskip 6\p@ \@minus 3\p@
    \let\@listi\@listI
  }%
\fi
\if@ll
  \newcommand\scriptsize{\@setfontsize\scriptsize\@viipt{8\p@}}
  \newcommand\tiny{\@setfontsize\tiny\@vpt{6\p@}}
  \newcommand\large{\@setfontsize\large\@xiipt{14\p@}}
  \newcommand\Large{\@setfontsize\Large\@xivpt{18\p@}}
  \newcommand\LARGE{\@setfontsize\LARGE\@xviipt{20\p@}}
  \newcommand\huge{\@setfontsize\huge\@xxpt{25\p@}}
  \newcommand\Huge{\@setfontsize\Huge\@xxvpt{30\p@}}
\else
  \def\scriptsize{\@setsize\scriptsize{8\p@}\viipt\@viipt}
  \def\tiny{\@setsize\tiny{6\p@}\vpt\@vpt}
  \def\large{\@setsize\large{14\p@}\xiipt\@xiipt}
  \def\Large{\@setsize\Large{18\p@}\xivpt\@xivpt}
  \def\LARGE{\@setsize\LARGE{20\p@}\xviipt\@xviipt}
  \def\huge{\@setsize\huge{25\p@}\xxpt\@xxpt}
  \def\Huge{\@setsize\Huge{30\p@}\xxvpt\@xxvpt}
\fi
\normalsize

% make aubox hsize/number of authors up to 3, less gutter
% then showbox gutter showbox gutter showbox -- GKMT Aug 99
\newbox\@acmtitlebox
\def\@maketitle{\newpage
 \null
 \setbox\@acmtitlebox\vbox{%
\baselineskip 20pt
\vskip 2em                   % Vertical space above title.
   \begin{center}
    {\ttlfnt \@title\par}       % Title set in 18pt Helvetica (Arial) bold size.
    \vskip 1.5em                % Vertical space after title.
%This should be the subtitle.
{\subttlfnt \the\subtitletext\par}\vskip 1.25em%\fi
    {\baselineskip 16pt\aufnt   % each author set in \12 pt Arial, in a
     \lineskip .5em             % tabular environment
     \begin{tabular}[t]{c}\@author
     \end{tabular}\par}
    \vskip 1.5em               % Vertical space after author.
   \end{center}}
 \dimen0=\ht\@acmtitlebox
 \advance\dimen0 by -12.75pc\relax % Increased space for title box -- KBT
 \unvbox\@acmtitlebox
 \ifdim\dimen0<0.0pt\relax\vskip-\dimen0\fi}


\newcount\titlenotecount
\global\titlenotecount=0
\newtoks\tntoks
\newtoks\tntokstwo
\newtoks\tntoksthree
\newtoks\tntoksfour
\newtoks\tntoksfive

\def\abstract{
\ifnum\titlenotecount>0 % was =1
    \insert\footins{%
    \reset@font\footnotesize
        \interlinepenalty\interfootnotelinepenalty
        \splittopskip\footnotesep
        \splitmaxdepth \dp\strutbox \floatingpenalty \@MM
        \hsize\columnwidth \@parboxrestore
        \protected@edef\@currentlabel{%
        }%
        \color@begingroup
\ifnum\titlenotecount=1
      \@maketntext{%
         \raisebox{4pt}{$\ast$}\rule\z@\footnotesep\ignorespaces\the\tntoks\@finalstrut\strutbox}%
\fi
\ifnum\titlenotecount=2
      \@maketntext{%
      \raisebox{4pt}{$\ast$}\rule\z@\footnotesep\ignorespaces\the\tntoks\par\@finalstrut\strutbox}%
\@maketntext{%
         \raisebox{4pt}{$\dagger$}\rule\z@\footnotesep\ignorespaces\the\tntokstwo\@finalstrut\strutbox}%
\fi
\ifnum\titlenotecount=3
      \@maketntext{%
         \raisebox{4pt}{$\ast$}\rule\z@\footnotesep\ignorespaces\the\tntoks\par\@finalstrut\strutbox}%
\@maketntext{%
         \raisebox{4pt}{$\dagger$}\rule\z@\footnotesep\ignorespaces\the\tntokstwo\par\@finalstrut\strutbox}%
\@maketntext{%
         \raisebox{4pt}{$\ddagger$}\rule\z@\footnotesep\ignorespaces\the\tntoksthree\@finalstrut\strutbox}%
\fi
\ifnum\titlenotecount=4
      \@maketntext{%
         \raisebox{4pt}{$\ast$}\rule\z@\footnotesep\ignorespaces\the\tntoks\par\@finalstrut\strutbox}%
\@maketntext{%
         \raisebox{4pt}{$\dagger$}\rule\z@\footnotesep\ignorespaces\the\tntokstwo\par\@finalstrut\strutbox}%
\@maketntext{%
         \raisebox{4pt}{$\ddagger$}\rule\z@\footnotesep\ignorespaces\the\tntoksthree\par\@finalstrut\strutbox}%
\@maketntext{%
         \raisebox{4pt}{$\S$}\rule\z@\footnotesep\ignorespaces\the\tntoksfour\@finalstrut\strutbox}%
\fi
\ifnum\titlenotecount=5
      \@maketntext{%
         \raisebox{4pt}{$\ast$}\rule\z@\footnotesep\ignorespaces\the\tntoks\par\@finalstrut\strutbox}%
\@maketntext{%
         \raisebox{4pt}{$\dagger$}\rule\z@\footnotesep\ignorespaces\the\tntokstwo\par\@finalstrut\strutbox}%
\@maketntext{%
         \raisebox{4pt}{$\ddagger$}\rule\z@\footnotesep\ignorespaces\the\tntoksthree\par\@finalstrut\strutbox}%
\@maketntext{%
         \raisebox{4pt}{$\S$}\rule\z@\footnotesep\ignorespaces\the\tntoksfour\par\@finalstrut\strutbox}%
\@maketntext{%
         \raisebox{4pt}{$\P$}\rule\z@\footnotesep\ignorespaces\the\tntoksfive\@finalstrut\strutbox}%
\fi
   \color@endgroup} %g}
\fi
\setcounter{footnote}{0}
\section*{ABSTRACT}\normalsize%\ninept
}

\def\endabstract{\if@twocolumn\else\endquotation\fi}

\def\keywords{\if@twocolumn
\section*{Keywords}
\else \small
\quotation
\fi}

\def\terms{\if@twocolumn
\section*{General Terms}
\else \small
\quotation
\fi}

% -- Classification needs to be a bit smart due to optionals - Gerry/Georgia November 2nd. 1999
\newcount\catcount
\global\catcount=1

\def\category#1#2#3{%
\ifnum\catcount=1
\section*{Categories and Subject Descriptors}
\advance\catcount by 1\else{\unskip; }\fi
    \@ifnextchar [{\@category{#1}{#2}{#3}}{\@category{#1}{#2}{#3}[]}%
}

\def\@category#1#2#3[#4]{%
    \begingroup
        \let\and\relax
            #1 [\textbf{#2}]%
            \if!#4!%
                \if!#3!\else : #3\fi
            \else
                :\space
                \if!#3!\else #3\kern\z@---\hskip\z@\fi
                \textit{#4}%
            \fi
    \endgroup
}
%

%%% This section (written by KBT) handles the 1" box in the lower left
%%% corner of the left column of the first page by creating a picture,
%%% and inserting the predefined string at the bottom (with a negative
%%% displacement to offset the space allocated for a non-existent
%%% caption).
%%%
\newtoks\copyrightnotice
\def\ftype@copyrightbox{8}
\def\@copyrightspace{
\@float{copyrightbox}[b]
\begin{center}
\setlength{\unitlength}{1pc}
\begin{picture}(20,6) %Space for copyright notice
\put(0,-0.95){\crnotice{\@toappear}}
\end{picture}
\end{center}
\end@float}

\def\@toappear{} % Default setting blank - commands below change this.
\long\def\toappear#1{\def\@toappear{\parbox[b]{20pc}{\baselineskip 9pt#1}}}
\def\toappearbox#1{\def\@toappear{\raisebox{5pt}{\framebox[20pc]{\parbox[b]{19pc}{#1}}}}}

\newtoks\conf
\newtoks\confinfo
\def\conferenceinfo#1#2{\global\conf={#1}\global\confinfo{#2}}


%\def\marginpar{\@latexerr{The \marginpar command is not allowed in the
%  `acmconf' document style.}\@eha}

\def\marginpar{\ClassError{%
    \string\marginpar\space is not allowed in the `acmconf' document		% January 2008
    style}\@eha}

\mark{{}{}}     % Initializes TeX's marks

\def\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}

\def\@begintheorem#1#2{%
    \parskip 0pt % GM July 2000 (for tighter spacing)
    \trivlist
    \item[%
        \hskip 10\p@
        \hskip \labelsep
        {{\sc #1}\hskip 5\p@\relax#2.}%
    ]
    \it
}
\def\@opargbegintheorem#1#2#3{%
    \parskip 0pt % GM July 2000 (for tighter spacing)
    \trivlist
    \item[%
        \hskip 10\p@
        \hskip \labelsep
        {\sc #1\ #2\             % This mod by Gerry to enumerate corollaries
   \setbox\@tempboxa\hbox{(#3)}  % and bracket the 'corollary title'
        \ifdim \wd\@tempboxa>\z@ % and retain the correct numbering of e.g. theorems
            \hskip 5\p@\relax    % if they occur 'around' said corollaries.
            \box\@tempboxa       % Gerry - Nov. 1999.
        \fi.}%
    ]
    \it
}
\newif\if@qeded
\global\@qededfalse

% -- original
%\def\proof{%
%  \vspace{-\parskip} % GM July 2000 (for tighter spacing)
%    \global\@qededfalse
%    \@ifnextchar[{\@xproof}{\@proof}%
%}
% -- end of original

% (JSS) Fix for vertical spacing bug - Gerry Murray July 30th. 2002
\def\proof{%
\vspace{-\lastskip}\vspace{-\parsep}\penalty-51%
\global\@qededfalse
\@ifnextchar[{\@xproof}{\@proof}%
}

\def\endproof{%
    \if@qeded\else\qed\fi
    \endtrivlist
}
\def\@proof{%
    \trivlist
    \item[%
        \hskip 10\p@
        \hskip \labelsep
        {\sc Proof.}%
    ]
    \ignorespaces
}
\def\@xproof[#1]{%
    \trivlist
    \item[\hskip 10\p@\hskip \labelsep{\sc Proof #1.}]%
    \ignorespaces
}
\def\qed{%
    \unskip
    \kern 10\p@
    \begingroup
        \unitlength\p@
        \linethickness{.4\p@}%
        \framebox(6,6){}%
    \endgroup
    \global\@qededtrue
}

\def\newdef#1#2{%
    \expandafter\@ifdefinable\csname #1\endcsname
        {\@definecounter{#1}%
         \expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
         \global\@namedef{#1}{\@defthm{#1}{#2}}%
         \global\@namedef{end#1}{\@endtheorem}%
    }%
}
\def\@defthm#1#2{%
    \refstepcounter{#1}%
    \@ifnextchar[{\@ydefthm{#1}{#2}}{\@xdefthm{#1}{#2}}%
}
\def\@xdefthm#1#2{%
    \@begindef{#2}{\csname the#1\endcsname}%
    \ignorespaces
}
\def\@ydefthm#1#2[#3]{%
    \trivlist
    \item[%
        \hskip 10\p@
        \hskip \labelsep
        {\it #2%
%         \savebox\@tempboxa{#3}%
         \saveb@x\@tempboxa{#3}%		% January 2008
         \ifdim \wd\@tempboxa>\z@
            \ \box\@tempboxa
         \fi.%
        }]%
    \ignorespaces
}
\def\@begindef#1#2{%
    \trivlist
    \item[%
        \hskip 10\p@
        \hskip \labelsep
        {\it #1\ \rm #2.}%
    ]%
}
\def\theequation{\arabic{equation}}

\newcounter{part}
\newcounter{section}
\newcounter{subsection}[section]
\newcounter{subsubsection}[subsection]
\newcounter{paragraph}[subsubsection]
\def\thepart{\Roman{part}}
\def\thesection{\arabic{section}}
\def\thesubsection{\thesection.\arabic{subsection}}
\def\thesubsubsection{\thesubsection.\arabic{subsubsection}} %removed \subsecfnt 29 July 2002 gkmt
\def\theparagraph{\thesubsubsection.\arabic{paragraph}} %removed \subsecfnt 29 July 2002 gkmt
\newif\if@uchead
\@ucheadfalse

%% CHANGES: NEW NOTE
%% NOTE: OK to use old-style font commands below, since they were
%% suitably redefined for LaTeX2e
%% END CHANGES
\setcounter{secnumdepth}{3}
\def\part{%
    \@startsection{part}{9}{\z@}{-10\p@ \@plus -4\p@ \@minus -2\p@}
        {4\p@}{\normalsize\@ucheadtrue}%
}
\def\section{%
    \@startsection{section}{1}{\z@}{-10\p@ \@plus -4\p@ \@minus -2\p@}% GM
    {4\p@}{\baselineskip 14pt\secfnt\@ucheadtrue}%
}

\def\subsection{%
    \@startsection{subsection}{2}{\z@}{-8\p@ \@plus -2\p@ \@minus -\p@}
    {4\p@}{\secfnt}%
}
\def\subsubsection{%
    \@startsection{subsubsection}{3}{\z@}{-8\p@ \@plus -2\p@ \@minus -\p@}%
    {4\p@}{\subsecfnt}%
}
%\def\paragraph{%
%    \vskip 12pt\@startsection{paragraph}{3}{\z@}{6\p@ \@plus \p@}% original
%    {-5\p@}{\subsecfnt}%
%}
%  If one wants sections, subsections and subsubsections numbered,
%  but not paragraphs, one usually sets secnumepth to 3.
%  For that, the "depth" of paragraphs must be given correctly
%  in the definition (``4'' instead of ``3'' as second argument
%  of @startsection):
\def\paragraph{%
    \vskip 12pt\@startsection{paragraph}{4}{\z@}{6\p@ \@plus \p@}%    % GM and Wolfgang May - 11/30/06
    {-5\p@}{\subsecfnt}%
}
\let\@period=.
\def\@startsection#1#2#3#4#5#6{%
        \if@noskipsec  %gkmt, 11 aug 99
        \global\let\@period\@empty
        \leavevmode
        \global\let\@period.%
    \fi
      \par %
    \@tempskipa #4\relax
    \@afterindenttrue
    \ifdim \@tempskipa <\z@
        \@tempskipa -\@tempskipa
        \@afterindentfalse
    \fi
    \if@nobreak
    \everypar{}%
    \else
        \addpenalty\@secpenalty
        \addvspace\@tempskipa
    \fi
\parskip=0pt % GM July 2000 (non numbered) section heads
    \@ifstar
        {\@ssect{#3}{#4}{#5}{#6}}
        {\@dblarg{\@sect{#1}{#2}{#3}{#4}{#5}{#6}}}%
}
\def\@sect#1#2#3#4#5#6[#7]#8{%
    \ifnum #2>\c@secnumdepth
        \let\@svsec\@empty
    \else
        \refstepcounter{#1}%
        \edef\@svsec{%
            \begingroup
                %\ifnum#2>2 \noexpand\rm \fi % changed to next 29 July 2002 gkmt
            \ifnum#2>2 \noexpand#6 \fi
                \csname the#1\endcsname
            \endgroup
            \ifnum #2=1\relax .\fi
            \hskip 1em
        }%
    \fi
    \@tempskipa #5\relax
    \ifdim \@tempskipa>\z@
        \begingroup
            #6\relax
            \@hangfrom{\hskip #3\relax\@svsec}%
            \begingroup
                \interlinepenalty \@M
                \if@uchead
                    \uppercase{#8}%
                \else
                    #8%
                \fi
                \par
            \endgroup
        \endgroup
        \csname #1mark\endcsname{#7}%
        \vskip -12pt  %gkmt, 11 aug 99 and GM July 2000 (was -14) - numbered section head spacing
\addcontentsline{toc}{#1}{%
            \ifnum #2>\c@secnumdepth \else
                \protect\numberline{\csname the#1\endcsname}%
            \fi
            #7%
        }%
    \else
        \def\@svsechd{%
            #6%
            \hskip #3\relax
            \@svsec
            \if@uchead
                \uppercase{#8}%
            \else
                #8%
            \fi
            \csname #1mark\endcsname{#7}%
            \addcontentsline{toc}{#1}{%
                \ifnum #2>\c@secnumdepth \else
                    \protect\numberline{\csname the#1\endcsname}%
                \fi
                #7%
            }%
        }%
    \fi
    \@xsect{#5}\hskip 1pt
    \par
}
\def\@xsect#1{%
    \@tempskipa #1\relax
    \ifdim \@tempskipa>\z@
        \par
        \nobreak
        \vskip \@tempskipa
        \@afterheading
    \else
        \global\@nobreakfalse
        \global\@noskipsectrue
        \everypar{%
            \if@noskipsec
                \global\@noskipsecfalse
                \clubpenalty\@M
                \hskip -\parindent
                \begingroup
                    \@svsechd
                    \@period
                \endgroup
                \unskip
                \@tempskipa #1\relax
                \hskip -\@tempskipa
            \else
                \clubpenalty \@clubpenalty
                \everypar{}%
            \fi
        }%
    \fi
    \ignorespaces
}
\def\@trivlist{%
    \@topsepadd\topsep
    \if@noskipsec
        \global\let\@period\@empty
        \leavevmode
        \global\let\@period.%
    \fi
    \ifvmode
        \advance\@topsepadd\partopsep
    \else
        \unskip
        \par
    \fi
    \if@inlabel
        \@noparitemtrue
        \@noparlisttrue
    \else
        \@noparlistfalse
        \@topsep\@topsepadd
    \fi
    \advance\@topsep \parskip
    \leftskip\z@skip
    \rightskip\@rightskip
    \parfillskip\@flushglue
    \@setpar{\if@newlist\else{\@@par}\fi}
    \global\@newlisttrue
    \@outerparskip\parskip
}

%%% Actually, 'abbrev' works just fine as the default
%%% Bibliography style.

\typeout{Using 'Abbrev' bibliography style}
\newcommand\bibyear[2]{%
    \unskip\quad\ignorespaces#1\unskip
    \if#2..\quad \else \quad#2 \fi
}
\newcommand{\bibemph}[1]{{\em#1}}
\newcommand{\bibemphic}[1]{{\em#1\/}}
\newcommand{\bibsc}[1]{{\sc#1}}
\def\@normalcite{%
    \def\@cite##1##2{[##1\if@tempswa , ##2\fi]}%
}
\def\@citeNB{%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi}%
}
\def\@citeRB{%
    \def\@cite##1##2{##1\if@tempswa , ##2\fi]}%
}
\def\start@cite#1#2{%
    \edef\citeauthoryear##1##2##3{%
        ###1%
        \ifnum#2=\z@ \else\ ###2\fi
    }%
    \ifnum#1=\thr@@
        \let\@@cite\@citeyear
    \else
        \let\@@cite\@citenormal
    \fi
    \@ifstar{\@citeNB\@@cite}{\@normalcite\@@cite}%
}
%\def\cite{\start@cite23}
\DeclareRobustCommand\cite{\start@cite23}		% January 2008
\def\citeNP{\cite*}					% No Parentheses e.g. 5
%\def\citeA{\start@cite10}
\DeclareRobustCommand\citeA{\start@cite10}		% January 2008
\def\citeANP{\citeA*}
%\def\shortcite{\start@cite23}				
\DeclareRobustCommand\shortcite{\start@cite23}		% January 2008
\def\shortciteNP{\shortcite*}
%\def\shortciteA{\start@cite20}
\DeclareRobustCommand\shortciteA{\start@cite20}		% January 2008
\def\shortciteANP{\shortciteA*}
%\def\citeyear{\start@cite30}
\DeclareRobustCommand\citeyear{\start@cite30}		% January 2008
\def\citeyearNP{\citeyear*}
%\def\citeN{%
\DeclareRobustCommand\citeN{%				% January 2008
    \@citeRB
    \def\citeauthoryear##1##2##3{##1\ [##3%
        \def\reserved@a{##1}%
        \def\citeauthoryear####1####2####3{%
            \def\reserved@b{####1}%
            \ifx\reserved@a\reserved@b
                ####3%
            \else
                \errmessage{Package acmart Error: author mismatch
                         in \string\citeN^^J^^J%
                    See the acmart package documentation for explanation}%
            \fi
        }%
    }%
    \@ifstar\@citeyear\@citeyear
}
%\def\shortciteN{%
\DeclareRobustCommand\shortciteN{%			% January 2008
    \@citeRB
    \def\citeauthoryear##1##2##3{##2\ [##3%
        \def\reserved@a{##2}%
        \def\citeauthoryear####1####2####3{%
            \def\reserved@b{####2}%
            \ifx\reserved@a\reserved@b
                ####3%
            \else
                \errmessage{Package acmart Error: author mismatch
                         in \string\shortciteN^^J^^J%
                    See the acmart package documentation for explanation}%
            \fi
        }%
    }%
    \@ifstar\@citeyear\@citeyear  % GM July 2000
}

\def\@citenormal{%
    \@ifnextchar [{\@tempswatrue\@citex;}%
% original                 {\@tempswafalse\@citex,[]}% was ; Gerry 2/24/00
{\@tempswafalse\@citex[]}%  	% GERRY FIX FOR BABEL 3/20/2009
}

\def\@citeyear{%
    \@ifnextchar [{\@tempswatrue\@citex,}%
% original                  {\@tempswafalse\@citex,[]}%
{\@tempswafalse\@citex[]}%	%  GERRY FIX FOR BABEL 3/20/2009
}

\def\@citex#1[#2]#3{%
    \let\@citea\@empty
    \@cite{%
        \@for\@citeb:=#3\do{%
            \@citea
% original            \def\@citea{#1 }%
            \def\@citea{#1, }% 	% GERRY FIX FOR BABEL 3/20/2009 -- SO THAT YOU GET [1, 2] IN THE BODY TEXT
            \edef\@citeb{\expandafter\@iden\@citeb}%
            \if@filesw
                \immediate\write\@auxout{\string\citation{\@citeb}}%
            \fi
            \@ifundefined{b@\@citeb}{%
                {\bf ?}%
                \@warning{%
                    Citation `\@citeb' on page \thepage\space undefined%
                }%
            }%
            {\csname b@\@citeb\endcsname}%
        }%
    }{#2}%
}
%\let\@biblabel\@gobble   % Dec. 2008 - Gerry
% ----
\def\@biblabelnum#1{[#1]} % Gerry's solution #1 - for Natbib -- April 2009
\let\@biblabel=\@biblabelnum  % Gerry's solution #1 - for Natbib -- April 2009
\def\newblock{\relax} % Gerry Dec. 2008
% ---
\newdimen\bibindent
\setcounter{enumi}{1}
\bibindent=0em
\def\thebibliography#1{% 
\ifnum\addauflag=0\addauthorsection\global\addauflag=1\fi
     \section[References]{%    <=== OPTIONAL ARGUMENT ADDED HERE
        {References} % was uppercased but this affects pdf bookmarks (SP/GM October 2004)
          {\vskip -9pt plus 1pt} % GM Nov. 2006 / GM July 2000 (for somewhat tighter spacing) 
         \@mkboth{{\refname}}{{\refname}}%
     }%
     \list{[\arabic{enumi}]}{%
         \settowidth\labelwidth{[#1]}%
         \leftmargin\labelwidth
         \advance\leftmargin\labelsep
         \advance\leftmargin\bibindent
         \parsep=0pt\itemsep=1pt % GM July 2000
         \itemindent -\bibindent
         \listparindent \itemindent
         \usecounter{enumi}
     }%
     \let\newblock\@empty
     \raggedright % GM July 2000
     \sloppy
     \sfcode`\.=1000\relax
}


\gdef\balancecolumns
{\vfill\eject
\global\@colht=\textheight
\global\ht\@cclv=\textheight
}

\newcount\colcntr
\global\colcntr=0
%\newbox\savebox
\newbox\saveb@x				% January 2008

\gdef \@makecol {%
\global\advance\colcntr by 1
\ifnum\colcntr>2 \global\colcntr=1\fi
   \ifvoid\footins
     \setbox\@outputbox \box\@cclv
   \else
     \setbox\@outputbox \vbox{%
\boxmaxdepth \@maxdepth
       \@tempdima\dp\@cclv
       \unvbox \@cclv
       \vskip-\@tempdima
       \vskip \skip\footins
       \color@begingroup
         \normalcolor
         \footnoterule
         \unvbox \footins
       \color@endgroup
       }%
   \fi
   \xdef\@freelist{\@freelist\@midlist}%
   \global \let \@midlist \@empty
   \@combinefloats
   \ifvbox\@kludgeins
     \@makespecialcolbox
   \else
     \setbox\@outputbox \vbox to\@colht {%
\@texttop
       \dimen@ \dp\@outputbox
       \unvbox \@outputbox
   \vskip -\dimen@
       \@textbottom
       }%
   \fi
   \global \maxdepth \@maxdepth
}
\def\titlenote{\@ifnextchar[\@xtitlenote{\stepcounter\@mpfn
\global\advance\titlenotecount by 1
\ifnum\titlenotecount=1
    \raisebox{9pt}{$\ast$}
\fi
\ifnum\titlenotecount=2
    \raisebox{9pt}{$\dagger$}
\fi
\ifnum\titlenotecount=3
    \raisebox{9pt}{$\ddagger$}
\fi
\ifnum\titlenotecount=4
\raisebox{9pt}{$\S$}
\fi
\ifnum\titlenotecount=5
\raisebox{9pt}{$\P$}
\fi
         \@titlenotetext
}}

\long\def\@titlenotetext#1{\insert\footins{%
\ifnum\titlenotecount=1\global\tntoks={#1}\fi
\ifnum\titlenotecount=2\global\tntokstwo={#1}\fi
\ifnum\titlenotecount=3\global\tntoksthree={#1}\fi
\ifnum\titlenotecount=4\global\tntoksfour={#1}\fi
\ifnum\titlenotecount=5\global\tntoksfive={#1}\fi
    \reset@font\footnotesize
    \interlinepenalty\interfootnotelinepenalty
    \splittopskip\footnotesep
    \splitmaxdepth \dp\strutbox \floatingpenalty \@MM
    \hsize\columnwidth \@parboxrestore
    \protected@edef\@currentlabel{%
    }%
    \color@begingroup
   \color@endgroup}}

%%%%%%%%%%%%%%%%%%%%%%%%%
\ps@plain
\baselineskip=11pt
\let\thepage\relax % For NO page numbers - GM Nov. 30th. 1999 and July 2000
\def\setpagenumber#1{\global\setcounter{page}{#1}}
%\pagenumbering{arabic}  % Arabic page numbers GM July 2000
\twocolumn             % Double column.
\flushbottom           % Even bottom -- alas, does not balance columns at end of document
\pagestyle{plain}

% Need Copyright Year and Copyright Data to be user definable (in .tex file).
% Gerry Nov. 30th. 1999
\newtoks\copyrtyr
\newtoks\acmcopyr
\newtoks\boilerplate
\global\acmcopyr={X-XXXXX-XX-X/XX/XX}  % Default - 5/11/2001 *** Gerry
\global\copyrtyr={20XX}                % Default - 3/3/2003 *** Gerry
\def\CopyrightYear#1{\global\copyrtyr{#1}}
\def\crdata#1{\global\acmcopyr{#1}}
\def\permission#1{\global\boilerplate{#1}}
%
\global\boilerplate={Permission to make digital or hard copies of all or part of this work for personal or classroom use is granted without fee provided that copies are not made or distributed for profit or commercial advantage and that copies bear this notice and the full citation on the first page.  To copy otherwise, to republish, to post on servers or to redistribute to lists, requires prior specific permission and/or a fee.}
\newtoks\copyrightetc
\global\copyrightetc{Copyright \the\copyrtyr\ ACM \the\acmcopyr\ ...\$10.00}
\toappear{\the\boilerplate\par
{\confname{\the\conf}} \the\confinfo\par \the\copyrightetc.}
%\DeclareFixedFont{\altcrnotice}{OT1}{tmr}{m}{n}{8}  % << patch needed for accenting e.g. Montreal - Gerry, May 2007
%\DeclareFixedFont{\altconfname}{OT1}{tmr}{m}{it}{8}  % << patch needed for accenting in italicized confname - Gerry, May 2007
%
%{\altconfname{{\the\conf}}} {\altcrnotice\the\confinfo\par} \the\copyrightetc.}  % << Gerry, May 2007
%
% The following section (i.e. 3 .sty inclusions) was added in May 2007 so as to fix the problems that many
% authors were having with accents. Sometimes accents would occur, but the letter-character would be of a different
% font. Conversely the letter-character font would be correct but, e.g. a 'bar' would appear superimposed on the
% character instead of, say, an unlaut/diaresis. Sometimes the letter-character would NOT appear at all.
% Using [T1]{fontenc} outright was not an option as this caused 99% of the authors to 'produce' a Type-3 (bitmapped)
% PDF file - useless for production. 
%
% For proper (font) accenting we NEED these packages to be part of the .cls file i.e. 'ae', 'aecompl' and 'aeguil' 
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% This is file `ae.sty' 
\def\fileversion{1.3}
\def\filedate{2001/02/12}
\NeedsTeXFormat{LaTeX2e}
%\ProvidesPackage{ae}[\filedate\space\fileversion\space  % GM
% Almost European Computer Modern]                       % GM - keeping the log file clean(er)
\newif\if@ae@slides \@ae@slidesfalse
\DeclareOption{slides}{\@ae@slidestrue}
\ProcessOptions
\fontfamily{aer}
\RequirePackage[T1]{fontenc}
\if@ae@slides
    \renewcommand{\sfdefault}{laess}
    \renewcommand{\rmdefault}{laess} % no roman
    \renewcommand{\ttdefault}{laett}
\else
    \renewcommand{\sfdefault}{aess}
    \renewcommand{\rmdefault}{aer}
    \renewcommand{\ttdefault}{aett}
\fi
\endinput
%% 
%% End of file `ae.sty'.
%
%
\def\fileversion{0.9}
\def\filedate{1998/07/23}
\NeedsTeXFormat{LaTeX2e}
%\ProvidesPackage{aecompl}[\filedate\space\fileversion\space   % GM
%T1 Complements for AE fonts (D. Roegel)]                      % GM -- keeping the log file clean(er)
 
\def\@ae@compl#1{{\fontencoding{T1}\fontfamily{cmr}\selectfont\symbol{#1}}}
\def\guillemotleft{\@ae@compl{19}}
\def\guillemotright{\@ae@compl{20}}
\def\guilsinglleft{\@ae@compl{14}}
\def\guilsinglright{\@ae@compl{15}}
\def\TH{\@ae@compl{222}}
\def\NG{\@ae@compl{141}}
\def\ng{\@ae@compl{173}}
\def\th{\@ae@compl{254}}
\def\DJ{\@ae@compl{208}}
\def\dj{\@ae@compl{158}}
\def\DH{\@ae@compl{208}}
\def\dh{\@ae@compl{240}}
\def\@perthousandzero{\@ae@compl{24}}
\def\textperthousand{\%\@perthousandzero}
\def\textpertenthousand{\%\@perthousandzero\@perthousandzero}
\endinput
%
%
%% This is file `aeguill.sty' 
% This file gives french guillemets (and not guillemots!)
% built with the Polish CMR fonts (default), WNCYR fonts, the LASY fonts 
% or with the EC fonts. 
% This is useful in conjunction with the ae package
% (this package loads the ae package in case it has not been loaded)
%  and with or without the french(le) package.
%
% In order to get the guillemets, it is necessary to either type
% \guillemotleft and \guillemotright, or to use an 8 bit encoding
% (such as ISO-Latin1) which selects these two commands, 
% or, if you use the french package (but not the frenchle package), 
% to type << or >>.
%
% By default, you get the Polish CMR guillemets; if this package is loaded
% with the `cm' option, you get the LASY guillemets; with `ec,' you
% get the EC guillemets, and with `cyr,' you get the cyrillic guillemets.
%
% In verbatim mode, you always get the EC/TT guillemets.
%
% The default option is interesting in conjunction with PDF,
% because there is a Type 1 version of the Polish CMR fonts
% and these guillemets are very close in shape to the EC guillemets.
% There are no free Type 1 versions of the EC fonts.
%
% Support for Polish CMR guillemets was kindly provided by 
% Rolf Niepraschk <niepraschk@ptb.de> in version 0.99 (2000/05/22).
% Bernd Raichle provided extensive simplifications to the code
% for version 1.00.
%
% This package is released under the LPPL.
%
% Changes:
%   Date        version
%   2001/04/12  1.01    the frenchle and french package are now distinguished.
%
\def\fileversion{1.01}
\def\filedate{2001/04/12}
\NeedsTeXFormat{LaTeX2e}
%\ProvidesPackage{aeguill}[2001/04/12 1.01 %    % GM
%AE fonts with french guillemets (D. Roegel)]   % GM - keeping the log file clean(er)
%\RequirePackage{ae}  % GM May 2007 - already embedded here

\newcommand{\@ae@switch}[4]{#4}
\DeclareOption{ec}{\renewcommand\@ae@switch[4]{#1}}
\DeclareOption{cm}{\renewcommand\@ae@switch[4]{#2}}
\DeclareOption{cyr}{\renewcommand\@ae@switch[4]{#3}}
\DeclareOption{pl}{\renewcommand\@ae@switch[4]{#4}}
\ExecuteOptions{pl}
\ProcessOptions

%
% Load necessary packages
%
\@ae@switch{% ec
  % do nothing
}{% cm
  \RequirePackage{latexsym}%  GM - May 2007 - already 'mentioned as required' up above
}{% cyr
  \RequirePackage[OT2,T1]{fontenc}%
}{% pl
  \RequirePackage[OT4,T1]{fontenc}%
}

% The following command will be compared to \frenchname,
% as defined in french.sty and frenchle.sty.
\def\aeguillfrenchdefault{french}%

\let\guill@verbatim@font\verbatim@font
\def\verbatim@font{\guill@verbatim@font\ecguills{cmtt}%
                   \let\guillemotleft\@oguills\let\guillemotright\@fguills}

\begingroup \catcode`\<=13 \catcode`\>=13
\def\x{\endgroup
 \def\ae@lfguill{<<}%
 \def\ae@rfguill{>>}%
}\x

\newcommand{\ecguills}[1]{%
  \def\selectguillfont{\fontencoding{T1}\fontfamily{#1}\selectfont}%
  \def\@oguills{{\selectguillfont\symbol{19}}}%
  \def\@fguills{{\selectguillfont\symbol{20}}}%
  } 

\newcommand{\aeguills}{%
  \ae@guills
  % We redefine \guillemotleft and \guillemotright
  % in order to catch them when they are used 
  % with \DeclareInputText (in latin1.def for instance)
  % We use \auxWARNINGi as a safe indicator that french.sty is used.
  \gdef\guillemotleft{\ifx\auxWARNINGi\undefined
                         \@oguills % neither french.sty nor frenchle.sty
                      \else
                         \ifx\aeguillfrenchdefault\frenchname
                           \ae@lfguill  % french.sty
                         \else
                           \@oguills    % frenchle.sty
                         \fi
                      \fi}%
  \gdef\guillemotright{\ifx\auxWARNINGi\undefined
                         \@fguills % neither french.sty nor frenchle.sty
                       \else
                         \ifx\aeguillfrenchdefault\frenchname
                           \ae@rfguill  % french.sty
                         \else
                           \@fguills    % frenchle.sty
                         \fi
                       \fi}%
  }

%
% Depending on the class option
% define the internal command \ae@guills
\@ae@switch{% ec
  \newcommand{\ae@guills}{%
    \ecguills{cmr}}%
}{% cm
  \newcommand{\ae@guills}{%
    \def\selectguillfont{\fontencoding{U}\fontfamily{lasy}%
            \fontseries{m}\fontshape{n}\selectfont}%
    \def\@oguills{\leavevmode\nobreak
                \hbox{\selectguillfont (\kern-.20em(\kern.20em}\nobreak}%
    \def\@fguills{\leavevmode\nobreak
                \hbox{\selectguillfont \kern.20em)\kern-.2em)}%
                \ifdim\fontdimen\@ne\font>\z@\/\fi}}%
}{% cyr
  \newcommand{\ae@guills}{%
    \def\selectguillfont{\fontencoding{OT2}\fontfamily{wncyr}\selectfont}%
    \def\@oguills{{\selectguillfont\symbol{60}}}%
    \def\@fguills{{\selectguillfont\symbol{62}}}}
}{% pl
  \newcommand{\ae@guills}{%
    \def\selectguillfont{\fontencoding{OT4}\fontfamily{cmr}\selectfont}%
    \def\@oguills{{\selectguillfont\symbol{174}}}%
    \def\@fguills{{\selectguillfont\symbol{175}}}}
}


\AtBeginDocument{%
  \ifx\GOfrench\undefined
    \aeguills
  \else
    \let\aeguill@GOfrench\GOfrench
    \gdef\GOfrench{\aeguill@GOfrench \aeguills}%
  \fi
  }

\endinput
%


